Bordered Heegaard Floer homology: Invariance and pairing

We construct Heegaard Floer theory for 3-manifolds with connected boundary. The theory associates to an oriented, parametrized two-manifold a differential graded algebra. For a three-manifold with parametrized boundary, the invariant comes in two different versions, one of which (type D) is a module over the algebra and the other of which (type A) is an A-infinity module. Both are well-defined up to chain homotopy equivalence. For a decomposition of a 3-manifold into two pieces, the A-infinity tensor product of the type D module of one piece and the type A module from the other piece is HF^ of the glued manifold. As a special case of the construction, we specialize to the case of three-manifolds with torus boundary. This case can be used to give another proof of the surgery exact triangle for HF^. We relate the bordered Floer homology of a three-manifold with torus boundary with the knot Floer homology of a filling.

==> flip.tex <==
\makeatletter
\def\IfGraphicsFileExists#1#2#3{%
  \begingroup
  \let\input@path\Ginput@path
  \IfFileExists{#1}{#2}{#3}
  \endgroup
}

\newcommand\maybegraph[3][]{%
  \IfGraphicsFileExists{#2.#3}{\includegraphics[#1]{#2}}{}%
}

% Actually set the header/footer
\newcounter{tempcount}
\newcommand{\oddfootimage}{%
  \setcounter{tempcount}{\thepage/2}%
  \smash{\raisebox{14pt-\height}{\rlap{\maybegraph{flip-join-\thetempcount}{mps}}}}}

% The even images should perhaps be backwards, although it doesn't
% really matter for this sequence
\newcommand{\evenfootimage}{%
  \setcounter{tempcount}{\thepage/2-1}%
  \smash{\raisebox{14pt-\height}{\llap{\maybegraph{flip-split-\thetempcount}{mps}}}}}

\def\ps@flipheadings{\ps@empty
  \def\@evenhead{%
    \setTrue{runhead}%
    \normalfont\scriptsize
    \rlap{\thepage}\hfil
    \def\thanks{\protect\thanks@warning}%
    \leftmark{}{}\hfil}%
  \def\@oddhead{%
    \setTrue{runhead}%
    \normalfont\scriptsize \hfil
    \def\thanks{\protect\thanks@warning}%
    \rightmark{}{}\hfil \llap{\thepage}}%
  \let\@mkboth\markboth
  \def\@oddfoot{\hfil\oddfootimage}%
  \def\@evenfoot{\evenfootimage\hfil}%
}
\def\ps@flipplain{\ps@empty
  \def\@oddfoot{\normalfont\scriptsize\hfil\thepage\hfil\oddfootimage}%
  \def\@evenfoot{\normalfont\scriptsize\evenfootimage\hfil\thepage\hfil}}%
\def\ps@flipempty{\let\@mkboth\@gobbletwo
  \let\@oddhead\@empty \let\@evenhead\@empty
  \def\@oddfoot{\hfil\oddfootimage}%
  \def\@evenfoot{\evenfootimage\hfil}%
  \global\topskip\normaltopskip}
\footskip=14pt

\newcommand{\activateflip}{%
  \let\ps@plain\ps@flipplain
  \let\ps@empty\ps@flipempty
  \pagestyle{flipheadings}
}
\makeatother


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "InvPairing"
%%% End: 


==> glossary.tex <==
\setlength{\glstreeindent}{1em}
%\setlength{\glsdescwidth}{4em}
\setlength{\glsdescwidth}{6em}

\makeatletter
\newcommand{\minwidth}[2]{\leavevmode\setbox\@tempboxa\hbox{#2}%
  \@tempdima=#1\relax
  \ifdim\wd\@tempboxa>\@tempdima \usebox\@tempboxa
  \else \hbox to\@tempdima{\usebox\@tempboxa\hfil}\fi}

\newglossarystyle{hangtree}{%
  \renewenvironment{theglossary}%
    {\setlength{\parindent}{0pt}%
     \setlength{\parskip}{0pt plus 0.3pt}}%
    {}%
    \renewcommand{\glossarypreamble}{
      % \noindent
      % Notation is grouped logically, as follows. When used for more
      % than one purpose, notation may appear in more than one place.
      \begin{center}
      \begin{tabular}{ll}
        \textbf{General} & \pageref{gls:General}\\
        \textbf{$\Ainf$ structures} & \pageref{gls:ainfstr}\\
        \textbf{Algebra associated to a pointed matched circle} &
        \pageref{gls:algebrapmc}\\
        \textbf{Gradings} & \pageref{gls:Gradings}\\
        \textbf{Heegaard diagrams} & \pageref{gls:heegaarddiagrams}\\
        \textbf{Moduli spaces} & \pageref{gls:moduli}\\
        \textbf{Type $D$ modules} & \pageref{gls:TypeDMod}\\
        \textbf{Invariance of $\CFDa$} & \pageref{gls:DInvariance}\\
        \textbf{Type $A$ modules} & \pageref{gls:TypeAMod}\\
        \textbf{The pairing theorem} & \pageref{gls:Pairing}\\
        \textbf{Manifolds with torus boundary} & \pageref{gls:Torus}\\ 
        \textbf{Bimodules and change of framing} & \pageref{gls:Bimodules}\\
      \end{tabular}\end{center}
    }
  \renewcommand*{\glossaryheader}{}%
  \renewcommand*{\glsgroupheading}[1]{}%
  \renewcommand{\glossaryentryfield}[6]{%
    \hangindent0pt\relax
    \parindent0pt\relax
    \bigskip
%    \textbf{\glstarget{##1}{##2}}%
    \textbf{\glstarget{##1}{##2}}\phantomsection\protect\label{gls:##1}
    \ifx\relax##4\relax
    \else
      \space(##4)%
    \fi
    \par\nobreak}
  \renewcommand{\glossarysubentryfield}[6]{%
    \hangindent##1\glstreeindent\relax
    \advance\hangindent\glsdescwidth\relax
    \advance\hangindent\glstreeindent\relax
    \parindent\glstreeindent\relax
    \setlength{\@tempdimb}{\glsdescwidth}%
    \advance\@tempdimb##1\glstreeindent\relax
    \minwidth{\@tempdimb}{%
      \textbf{\glstarget{##2}{##3}}%
    \ifx\relax##5\relax
    \else
      \space(##5)%
    \fi
    \enspace}##4\glspostdescription\space ##6\par}%
  \renewcommand*{\glsgroupskip}{\indexspace}}
\renewcommand{\glossarymark}[1]{\@mkboth{\textsc{INDEX OF NOTATION}}{\textsc{INDEX OF NOTATION}}}
\makeatother

%General:

\newglossaryentry{General}
{
  name={General},
  description={\nopostdesc},
  sort=aaa
}
\newglossaryentry{Id}{
  name={\ensuremath{\Id}},
  description={Identity morphism},
  sort=Identity,
  parent=General
}
 \newglossaryentry{nset}{
   name={\ensuremath{[n]}},
   description={The set $\{1,\dots,n\}$},
   sort=nset,
   parent=General
 }
 \newglossaryentry{minus}{
   name={\ensuremath{-}},
   description={Orientation reversal},
   sort=minus,
   parent=General
 }
 \newglossaryentry{SymmDiff}{
   name={\ensuremath{\symmdiff}},
   description={The symmetric difference of two sets; $S\symmdiff
     T\coloneqq (S \setminus T) \cup (T \setminus S)$},
   sort=SymmDiff,
   parent=General
 }

%Gradings
\newglossaryentry{Gradings}
{
  name={Gradings},
  description={\nopostdesc}
}
\newglossaryentry{Glambda}{
  name={\ensuremath{(G,\lambda)}},
  description={Group with distinguished central element},
  sort=Glambda,
  parent=Gradings
}

\newglossaryentry{lessthan}{
  name={\ensuremath{<}},
  description={Partial order on a grading group or set given by $a<b$ if $b=\lambda^n a$ for some $n\in\NN$},
  sort=less,
  parent=Gradings
}


\newglossaryentry{gr}{
  name={\ensuremath{\gr}},
  description={Grading on group-graded differential algebra or module},
  sort=gr,
  parent=Gradings
}
\newglossaryentry{grTensorProd}{
  name={\ensuremath{\gr(m\otimes n)}},
  description={Grading on tensor product of modules},
  sort=grTensorProd,
  parent=gr
}
\newglossaryentry{grprime}{
  name={\ensuremath{\grb}},
  description={Grading in $G'(n)$ of element of $\Alg(\PMC)$; or
    $G'(4k)$-set grading on $\CFAa$ or $\CFDa$},
  sort=grprime,
  parent=gr
}
\newglossaryentry{tgrprime}{
  name={\ensuremath{\protect\underline{\gr}'}},
  description={$G'(4k)$-set grading on $\protect\tCFAa$ or $\protect\tCFDa$},
  sort=grprimet,
  parent=gr
}
\newglossaryentry{tgr}{
  name={\ensuremath{\protect\underline{\gr}}},
  description={$G(\PMC)$-set grading on $\protect\tCFAa$ or $\protect\tCFDa$},
  sort=grt,
  parent=gr
}
\newglossaryentry{grprimevecrho}{
  name={\ensuremath{\grb(\protect\vec{\rho})}},
  description={$\prod_{i=1}^n\grb(a(\rho_i))$},
  sort=grprimevecrho,
  parent=gr
}
\newglossaryentry{grprimevecrhos}{
  name={\ensuremath{\grb(\protect\vec{\rhos})}},
  description={$\prod_{i=1}^n\grb(a(\rhos_i))$},
  sort=grprimevecrhos,
  parent=gr
}
\newglossaryentry{smallgr}{
  name={\ensuremath{\gr}},
  description={$\smallGroup(\PMC)$-grading on $\Alg(\PMC)$; or
    $\smallGroup(\PMC)$-set grading on $\CFAa$ or $\CFDa$},
  sort=gr,
  parent=gr
}
\newglossaryentry{grBox}{
  name={\ensuremath{\grT}},
  description={Grading on $\CFAa\DT\CFDa$},
  sort=grTensorProductBox,
  parent=gr
}

\newglossaryentry{gbig}{
  name={\ensuremath{\gb(B)}},
  description={$(-e(B) - n_\x(B) - n_\y(B), \bdy^\bdy(B))$. Also given
  by $\lambda^{\ell-\ind(B,\vec{\rhos})} \prod_{i=1}^\ell
  \grb(a(\rhos_i))$ if $(B,\vec{\rhos})$ is compatible},
  sort=gbig,
  parent=Gradings
}
\newglossaryentry{gsmall}{
  name={\ensuremath{\gs(B)}},
  description={$\psi(I_A(\x))\gb(B)\psi(I_A(\y))^{-1}$},
  sort=gsmall,
  parent=Gradings
}

\newglossaryentry{DGAsubg}{
  name={\ensuremath{\DGA_g}},
  description={Part of $\DGA$ in grading $g$},
  sort=Asubg,
  parent=Gradings
}
\newglossaryentry{shiftV}{
  name={\ensuremath{V[n]}},
  description={Shift functor applied to $V$ ($\ZZ$-graded or $G$-graded
    sense)},
  sort=Vshift,
  parent=Gradings
}
% \newglossaryentry{ZShift}{
%   name={\ensuremath{M[n]}},
%   description={Shift functor applied to $M$ ($\ZZ$-graded sense)},
%   sort=ShiftZ,
%   parent=shiftV
% }
\newglossaryentry{Gsubs}{
  name={\ensuremath{G_s}},
  description={Stabilizer of $s$},
  sort=Gsubs,
  parent=Gradings
}
\newglossaryentry{GsubsCosets}{
  name={\ensuremath{G_s\protect\backslash G}},
  description={Right cosets of $G_s$},
  sort=GsubsCosets,
  parent=Gradings
}
\newglossaryentry{ProductGSets}{
  name={\ensuremath{S\times_GT}},
  description={Fiber product of $G$-sets},
  sort=ProductGSets,
  parent=Gradings
}
\newglossaryentry{Group}{
  name={\ensuremath{G}},
  description={A grading group},
  sort=G,
  parent=Gradings
}
\newglossaryentry{bigGroup}{
  name={\ensuremath{\bigGroup(n)}},
  description={Big grading group on $n$
  positions; $\ZZ\hookrightarrow \bigGroup(n)
   \twoheadrightarrow H_1(Z',\CircPts)$},
  sort=Gprime,
  parent=Group
}
\newglossaryentry{jalpha}{
  name={\ensuremath{(j,\alpha)}},
  description={Element of $\bigGroup(n)$; $j\in\OneHalf\ZZ$ is the Maslov
    component; $\alpha\in H_1(Z,\CircPts)$ is the $\SpinC$
    component},
  sort=jalpha,
  parent=Gradings
}
\newglossaryentry{biggpprod}{
  name={\ensuremath{(j_1,\alpha_1)\cdot(j_2,\alpha_2)}},
  description={$=(j_1 + j_2 +
    L(\alpha_1, \alpha_2), \alpha_1 + \alpha_2)$.
},
  sort=product,
  parent=jalpha
}

\newglossaryentry{smallGroup}{
  name={\ensuremath{\smallGroup(\PMC)}},
  description={Small grading group for $\PMC$; $\ZZ \hookrightarrow \smallGroup(n)
   \twoheadrightarrow H_1(F(\PMC))$},
  sort=Gsmall,
  parent=Group
}
\newglossaryentry{homola}{
  name={\ensuremath{[a]}},
  description={Homology class in $H_1(Z',\mathbf{a})$ of
    algebra element $a$},
  sort=abracs,
  parent=Gradings
}
\newglossaryentry{Hofalpha}{
  name={\ensuremath{\overline{\alpha}}},
  description={Element of $H_1(F(\PMC))$
  associated to appropriate element of $H_1(Z',\mathbf{a})$},
  sort=abracsalpha,
  parent=Gradings
}
\newglossaryentry{epsilonalpha}{
  name={\ensuremath{\epsilon(\alpha)}},
  description={One quarter the number of parity changes in~$\alpha$},
  sort=epsilonalpha,
  parent=Gradings
}
\newglossaryentry{multalphap}{
  name={\ensuremath{m(\alpha,p)}},
  description={Multiplicity of $p$ in $\alpha$},
  sort=malphap,
  parent=Gradings
}
\newglossaryentry{Linkingalpha}{
  name={\ensuremath{L(\alpha_1,\alpha_2)}},
  description={$m(\alpha_2,\bdy\alpha_1)$},
  sort=Linking,
  parent=Gradings
}
\newglossaryentry{Linkingrho}{
  name={\ensuremath{L(\rho_1,\rho_2)}},
  description={$L([\rho_1],[\rho_2])$},
  sort=Linkingrho,
  parent=Linkingalpha
}
\newglossaryentry{Linkingrhos}{
  name={\ensuremath{L(\rhos_1,\rhos_2)}},
  description={$L([\rhos_1],[\rhos_2])$},
  sort=Linkingrhos,
  parent=Linkingalpha
}
\newglossaryentry{connectinghom}{
  name={\ensuremath{\partial}},
  description={Connecting homomorphism
  $H_1(Z',\CircPts)\to H_0(\CircPts)$},
  sort=dpartial,
  parent=Gradings
}
\newglossaryentry{lambda}{
  name={\ensuremath{\lambda}},
  description={Distinguished central element of a grading group or, in
  particular, of $G'(n)$ or $G'(\PMC)$},
  sort=lambda,
  parent=Gradings
}
% \newglossaryentry{lambdaGprime}{
%   name={\ensuremath{\lambda}},
%   description={Central element of $G'(n)$},
%   parent=lambda
% }
\newglossaryentry{iota}{
  name={\ensuremath{\iota(a)}},
  description={Maslov component of grading of algebra element $a$},
  sort=iota,
  parent=Gradings
}
\newglossaryentry{iotarhos}{
  name={\ensuremath{\iota(\rhos)}},
  description={Shorthand for $\iota(a(\rhos))$. Given explicitly by $\sum_{\{\rho_1, \rho_2\}\subset \rhos}
      \abs{L(\rho_1,\rho_2)} - \frac{\abs{\rhos}}{2}$},
  sort=iotarhos,
  parent=iota
}
\newglossaryentry{iotavecrhos}{
  name={\ensuremath{\iota(\protect\vec\rhos)}},
  description={Maslov part $\sum_{i}\iota(\rhos_i)+\sum_{i<j}
  L(\rhos_i,\rhos_j)$ of
    $\grb(a(\rhos_1))\cdots\grb(a(\rhos_\ell))$},
  sort=iotavecrhos,
  parent=iota
}
\newglossaryentry{refinementdata}{
  name={\ensuremath{\psi(\SetS)=\psi(I(\SetS))}},
  description={Elements of $\bigGroup(4k)$ used to
  refine $\bigGroup(4k)$-grading to $\smallGroup(\PMC)$-grading},
  sort=refinementdata,
  parent=Gradings
}

\newglossaryentry{ABigGrSet}{
  name={\ensuremath{\ABigGrSet}},
  description={$\bigGroup(4k)$-grading set for $\CFAa$},
  sort=SpA,
  parent=Gradings
}
\newglossaryentry{ASmallGrSet}{
  name={\ensuremath{\ASmallGrSet}},
  description={$\smallGroup(\PMC)$-grading set for $\CFAa$},
  sort=SqA,
  parent=Gradings
}
\newglossaryentry{DBigGrSet}{
  name={\ensuremath{\DBigGrSet}},
  description={$\bigGroup(4k)$-grading set for $\CFDa$},
  sort=SpD,
  parent=Gradings
}
\newglossaryentry{DSmallGrSet}{
  name={\ensuremath{\DSmallGrSet}},
  description={$\smallGroup(\PMC)$-grading set for $\CFDa$},
  sort=SqD,
  parent=Gradings
}

\newglossaryentry{reverseOr}{
  name={\ensuremath{r}},
  description={Identity map $Z\to -Z$ (orientation-reversing)},
  sort=reverse,
  parent=Gradings
}
\newglossaryentry{reverseOrGp}{
  name={\ensuremath{R}},
  description={Map $\bigGroup(4k) \to \bigGroup(4k)$ or
    $\smallGroup(\PMC) \to \smallGroup(-\PMC)$ given by $R(j,\alpha) = (j, r_* (\alpha))$},
  sort=reverseR,
  parent=Gradings
}

\newglossaryentry{PiOfGamma}{
  name={\ensuremath{\Pi(\gamma)}},
  description={Projection $\smallGroup\slash R(P_2(\x_2))
\to \bigl\{\spinc\in\SpinC(Y)\mathbin{\big\lvert}
\spinc\vert_{Y_i}\cong\spinc_i, i=1,2\bigr\}$ gotten by modding-out
$\ZZ$-action},
  sort=Pi,
  parent=Gradings
}

\newglossaryentry{Pofx}{
  name={\ensuremath{P(\x)}},
  description={Subgroup of $\smallGroup(\PMC)$ given by $\{\gs(B)\mid B \in \pi_2(\x,\x)\}$},
  sort=Pofxprime,
  parent=Gradings
}
\newglossaryentry{Pprimeofx}{
  name={\ensuremath{P'(\x)}},
  description={Subgroup of $\bigGroup(4k)$ given by $\{\gb(B)\mid B \in \pi_2(\x,\x)\}$},
  sort=Pofxprime,
  parent=Gradings
}
\newglossaryentry{divis}{
  name={\ensuremath{\divis(c_1(\spinc))}},
  description={Divisibility of $c_1(\spinc)$},
  sort=divis,
  parent=Gradings
}


%A-infinity algebras
\newglossaryentry{ainfstr}
{
  name={$\Ainf$ structures},
  description={\nopostdesc},
  sort=ainf
}
\newglossaryentry{Ground}{
  name={\ensuremath{\Ground}},
  description={Ground ring, a sum of $\Field$'s},
  sort=Ground,
  parent=ainfstr
}
\newglossaryentry{cDGA}{
  name={\ensuremath{\cDGA}},
  description={An $\Ainf$ algebra. Also used for algebra associated to
  a surface},
  sort=A,
  parent=ainfstr
}
\newglossaryentry{A}{
  name={\ensuremath{A}},
  description={The $\Ground$-module underlying the
  $\Ainf$ algebra $\Alg$},
  sort=A,
  parent=cDGA
}
\newglossaryentry{Atensori}{
  name={\ensuremath{A^{\otimes i}}},
  description={The $i\th$ tensor power of $A$},
  sort=Atensor,
  parent=cDGA
}
\newglossaryentry{musubi}{
  name={\ensuremath{\mu_i}},
  description={The (higher) products on an $\Ainf$ algebra},
  sort=musubi,
  parent=ainfstr
}
\newglossaryentry{msubi}{
  name={\ensuremath{m_i}},
  description={The (higher) products on an $\Ainf$ module},
  sort=musubiModule,
  parent=ainfstr
}
\newglossaryentry{barm}{
  name={\ensuremath{\overline{m}}},
  description={Differential on bar resolution of
    an $\Ainf$ module $\cModule$ gotten by considering all $m_i$ at once},
  sort=musubiModuleBar,
  parent=ainfstr
}

\newglossaryentry{TensorA}{
  name={\ensuremath{\Tensor^*(\DGA)}},
  description={Tensor (bar) algebra on $A$},
  sort=TensorA,
  parent=ainfstr
}
\newglossaryentry{TensorPlusA}{
  name={\ensuremath{\Tensor^+(\DGA)}},
  description={Augmentation ideal in tensor algebra $\Tensor^*(\DGA)$},
  sort=TensorAPlus,
  parent=ainfstr
}
\newglossaryentry{barD}{
  name={\ensuremath{\widebar{D}}},
  description={Differential on bar (tensor) algebra of an $\Ainf$ algebra},
  sort=Dbar,
  parent=ainfstr
}


\newglossaryentry{cModule}{
  name={\ensuremath{\cModule}},
  description={An $\Ainf$ module},
  sort=Module,
  parent=ainfstr
}
\newglossaryentry{M}{
  name={\ensuremath{M}},
  description={The $\Ground$-module underlying an
    $\Ainf$ module $\cModule$},
  sort=M,
  parent=cModule
}
\newglossaryentry{barModule}{
  name={\ensuremath{\widebar{\cModule}}},
  description={Bar resolution of $\cModule$},
  sort=Mbar,
  parent=cModule
}
\newglossaryentry{barM}{
  name={\ensuremath{\widebar{M}}},
  description={Module underlying bar resolution of $\cModule$},
  sort=Mbar,
  parent=cModule
}

\newglossaryentry{cNodule}{
  name={\ensuremath{\cNodule}},
  description={\dg (resp.~$\Ainf$) module associated to type $D$ structure $N$ over a
    \dg (resp.~$\Ainf$) algebra},
  sort=Nodule,
  parent=ainfstr
}
% \newglossaryentry{cNoduleAinf}{
% %  name={\ensuremath{\cNodule}},
%   description={$\Ainf$ module associated to a type $D$ structure $N$ over an $\Ainf$ algebra},
%   sort=Nodule,
%   parent=cNodule
% }


\newglossaryentry{fsubi}{
  name={\ensuremath{\{f_i\}}},
  description={A morphism of $\Ainf$ modules},
  sort=fsubi,
  parent=ainfstr
}

\newglossaryentry{DTP}{
  name={\ensuremath{\protect\DTP}},
  description={The $\Ainf$ tensor product},
  sort=TensorProd,
  parent=ainfstr
}
\newglossaryentry{DTPfId}{
  name={\ensuremath{f\protect\DTP\Id}},
  description={The $\Ainf$ tensor product of $f$ with the
    identity map},
  sort=Morphism,
  parent=DTP
}
\newglossaryentry{DT}{
  name={\ensuremath{\DT}},
  description={Box tensor product, a smaller model for $\Ainf$ tensor product},
  sort=TensorProdSmall,
  parent=ainfstr
}
\newglossaryentry{DTdiff}{
  name={\ensuremath{\bdy^\DT}},
  description={Differential on $\DT$},
  sort=DTdiff,
  parent=DT
}
\newglossaryentry{DTphiId}{
  name={\ensuremath{\phi\DT\Id_N}},
  description={Box tensor product
  of a homomorphism with the identity on $N$},
  sort=DTphiId,
  parent=DT
}


\newglossaryentry{ddiff}{
  name={\ensuremath{\delta^1}},
  description={Structure map of type $D$ structure},
  sort=ddiff,
  parent=ainfstr
}
\newglossaryentry{ddiffk}{
  name={\ensuremath{\delta^k}},
  description={Iterate of structure map $\delta^1$ on a
  type $D$ structure},
  sort=ddiffk,
  parent=ddiff
}
\newglossaryentry{ddiffall}{
  name={\ensuremath{\delta}},
  description={Sum of all $\delta^k$ for a type $D$ structure. Also
    used for connecting homomorphism on $H_*$},
  sort=ddiffzall,
  parent=ddiff
}
\newglossaryentry{typedmap}{
  name={\ensuremath{\psi^1}},
  description={Homomorphism of type $D$ structures},
  sort=psi,
  parent=ddiff
}
\newglossaryentry{typedmapk}{
  name={\ensuremath{\psi^k}},
  description={Analogue of $\delta^k$ for a homomorphism of type $D$ structures},
  sort=psik,
  parent=ddiff
}
\newglossaryentry{typedmapall}{
  name={\ensuremath{\psi}},
  description={Analogue of $\delta$ for a homomorphism of type $D$ structures},
  sort=psizall,
  parent=ddiff
}


\newglossaryentry{typedstr}{
  name={\ensuremath{(N,\delta^1)}},
  description={A type $D$ structure},
  sort=Ndelta,
  parent=ainfstr
}


%Algebra associated to a pointed matched circle
\newglossaryentry{algebrapmc}
{
  name={Algebra associated to a pointed matched circle},
  description={\nopostdesc}
}
 \newglossaryentry{Ank}{
   name={\ensuremath{\Alg(n,k)}},
   description={Strands algebra on $n$ places and $k$
     strands},
   sort=Ank,
   parent=algebrapmc
 }
 \newglossaryentry{Algn}{
   name={\ensuremath{\Alg(n)}},
   description={Strands algebra on $n$ places,
     $\Alg(n)=\bigoplus_k\Alg(n,k)$},
   sort=Anz,
   parent=algebrapmc
 }
 \newglossaryentry{AlgPMC}{
   name={\ensuremath{\Alg(\PMC)}},
   description={Algebra associated to pointed matched circle $\PMC$. $\Alg(\PMC)\subset\Alg(4k)$},
   sort=APMC,
   parent=algebrapmc
 }
 \newglossaryentry{AlgPMCi}{
   name={\ensuremath{\Alg(\PMC,i)}},
   description={Summand of $\Alg(\PMC)$ with weight
    $i$. $\Alg(\PMC,i)\subset \Alg(4k,k+i)$},
   sort=APMCi,
   parent=AlgPMC
 }

 \newglossaryentry{twoline}{
   name={\ensuremath{\protect\strands{1&2&4}{5&3&4}}},
   description={Element of $\Alg(n,k)$
     given by partial permutation $1\mapsto 5,2\mapsto3, 4\mapsto4$},
   sort=notationtwoline,
   parent=algebrapmc
 }
 \newglossaryentry{graphicalnotation}{
  name={\ensuremath{\protect\mfigb{strands-0}}},
  description={Graphical notation for the algebra element $\protect\strands{1&2&4}{5&3&4}$},
   sort=notationgraphical,
   parent=twoline
 }
 \newglossaryentry{chordnotation}{
   name={\ensuremath{\protect\reebchords{1&2}{5&3}}},
   description={Consistent set of Reeb chords $\{[1,5],[2,3]\}$},
   sort=notationchords,
   parent=algebrapmc
 }
 \newglossaryentry{honestnotation}{
   name={\ensuremath{\protect\honestalg{1}{6}{4}}},
   description={Element of $\Alg(\PMC)$
     shown in Equation~\eqref{eq:genus-two-strands}},
   sort=notationhonest,
   parent=algebrapmc
 }


 \newglossaryentry{invnum}{
   name={\ensuremath{\inv(a)}},
   description={Number of inversions of element $a$ of $\Alg(n,k)$},
   sort=invnum,
   parent=algebrapmc
 }
 \newglossaryentry{invnumphi}{
   name={\ensuremath{\inv(\phi)}},
   description={Number of inversions of partial
  permutation $\phi$},
   sort=invphi,
   parent=invnum
 }
 \newglossaryentry{invset}{
   name={\ensuremath{\Inv(\phi)}},
   description={Set of inversions of partial permutation $\phi$},
   sort=invnum,
   parent=invnum
 }
 \newglossaryentry{resolvecross}{
   name={\ensuremath{\phi_\sigma}},
   description={Result of resolving crossing in $\phi$ corresponding to $\sigma$},
   sort=phi,
   parent=algebrapmc
 }


 \newglossaryentry{IdemAnkS}{
   name={\ensuremath{I(S)}},
   description={Idempotent in $\Alg(n,k)$ associated to set
  $S\subset[n]$, $|S|=k$},
   sort=IdemAnkS,
   parent=algebrapmc
 }
 \newglossaryentry{IdemPMCS}{
   name={\ensuremath{I(\SetS)}},
   description={Idempotent of
    $\Alg(\PMC)$ associated to set $\SetS$ of matched pairs},
   sort=IdemPMC,
   parent=algebrapmc
 } 
 \newglossaryentry{Idemnk}{
   name={\ensuremath{\Idem(n,k)}},
   description={Ring of idempotents in $\Alg(n,k)$},
   sort=Idemsnk,
   parent=algebrapmc
 }
 \newglossaryentry{IdemPMC}{
   name={\ensuremath{\Idem(\PMC)}},
   description={Ring of idempotents of $\Alg(\PMC)$},
   sort=IdemsPMC,
   parent=algebrapmc
 }
 \newglossaryentry{IdemPMCi}{
   name={\ensuremath{\Idem(\PMC,i)}},
   description={Summand of $\Idem(\PMC)$ with weight $i$},
   sort=IdemsPMCi,
   parent=IdemPMC
 }
 \newglossaryentry{Unit}{
   name={\ensuremath{\Unit}},
   description={Unit of $\Alg(\PMC)$},
   sort=IdemZ,
   parent=algebrapmc
 }


 \newglossaryentry{Circle}{
   name={\ensuremath{Z}},
   description={An oriented circle},
   sort=Z,
   parent=algebrapmc
 }
 \newglossaryentry{PMC}{
   name={\ensuremath{\PMC}},
   description={Pointed matched circle},
   sort=ZPMC,
   parent=algebrapmc
 }
 \newglossaryentry{CircPts}{
   name={\ensuremath{\CircPts}},
   description={$n$ points in an oriented circle},
   sort=a,
   parent=algebrapmc
 }
 \newglossaryentry{Matching}{
   name={\ensuremath{M}},
   description={Matching function of a matched circle},
   sort=M,
   parent=algebrapmc
 }
\newglossaryentry{pmcz}{
  name={\ensuremath{z}},
  description={Basepoint for pointed matched circle},
  sort=zpmc,
  parent=algebrapmc}

\newglossaryentry{SurfPMC}{
  name={\ensuremath{F(\PMC)}},
  description={Surface associated to pointed matched
    circle $\PMC$},
  sort=FSurfPMC,
  parent=algebrapmc}

\newglossaryentry{lessdot}{
  name={\ensuremath{\lessdot}},
  description={Ordering on $\CircPts$ induced by
    orientation on $Z$ and basepoint $z$},
  sort=lessdot,
  parent=algebrapmc}


 \newglossaryentry{ReebChord}{
   name={\ensuremath{\rho}},
   description={A Reeb chord in $Z$},
   sort=ReebChord,
   parent=algebrapmc
 }
 \newglossaryentry{InitialEndpt}{
   name={\ensuremath{\rho^-}},
   description={Initial endpoint of Reeb chord $\rho$},
   sort=ReebChordInitial,
   parent=ReebChord
 }
 \newglossaryentry{InitialInitialEndpt}{
   name={\ensuremath{\rho^{--}}},
   description={Initial endpoint of chord being
  glued to left of $\rho$},
   sort=ReebChordInitialInitial,
   parent=ReebChord
 }
 \newglossaryentry{TerminalEndpt}{
   name={\ensuremath{\rho^+}},
   description={Terminal endpoint of Reeb chord $\rho$},
   sort=ReebChordTerminal,
   parent=ReebChord
 }
 \newglossaryentry{TerminalTerminalEndpt}{
   name={\ensuremath{\rho^{++}}},
   description={Terminal endpoint of chord being
     glued to right of $\rho$},
   sort=ReebChordTerminalTerminal,
   parent=ReebChord
 }

 \newglossaryentry{ReebChords}{
   name={\ensuremath{\rhos}},
   description={A set of Reeb chords},
   sort=ReebChords,
   parent=algebrapmc
 }
 \newglossaryentry{InitialEndpts}{
   name={\ensuremath{\rhos^-}},
   description={Initial endpoints of set of Reeb chords $\rhos$},
   sort=ReebChordsInitial,
   parent=ReebChords
 }
 \newglossaryentry{TerminalEndpts}{
   name={\ensuremath{\rhos^+}},
   description={Terminal endpoints of set of Reeb chords $\rhos$},
   sort=ReebChordsTerminal,
   parent=ReebChords
 }
 \newglossaryentry{ReebChordsSeqSets}{
   name={\ensuremath{\protect\vec{\rhos}}},
   description={A sequence $(\rhos_1,\dots,\rhos_n)$ of sets of Reeb chords},
   sort=ReebChordsSeqSets,
   parent=algebrapmc
 }
 \newglossaryentry{ReebChordsSeqSetsOrRev}{
   name={\ensuremath{-\protect\vec{\rhos}}},
   description={Sequence obtained by reversing the orientation of each
   Reeb chord in $\vec{\rhos}$ (but keeping the same order)},
   sort=ReebChordsSeqSetsOrRev,
   parent=ReebChordsSeqSets
 }
 \newglossaryentry{ReebChordsSeqSetsInt}{
   name={\ensuremath{\protect\vec\rhos_{[i,j]}}},
   description={Subsequence $(\rhos_i,\dots,\rhos_j)$ of~$\protect\vec\rhos$},
   sort=ReebChordsSeqSetsInt,
   parent=ReebChordsSeqSets
 }
 \newglossaryentry{ConcatSeqs}{
   name={\ensuremath{(\protect\vec{\rhos},\protect\vec{\rhos}')}},
   description={Concatenation of the sequences $\vec{\rhos}$ and $\vec{\rhos}'$},
   sort=concat,
   parent=ReebChordsSeqSets
 }
 \newglossaryentry{ReebChordSeq}{
   name={\ensuremath{\protect\vec{\rho}}},
   description={A sequence $(\rho_1,\dots,\rho_n)$ of Reeb chords or sequence $(\{\rho_1\},\dots,\{\rho_n\})$ of singleton sets of Reeb chords},
   sort=ReebChordzSeq,
   parent=algebrapmc
 }
 \newglossaryentry{ReebChordSeqOrRev}{
   name={\ensuremath{-\protect\vec{\rho}}},
   description={The sequence $(-\rho_1,\dots,-\rho_n)$},
   sort=ReebChordSeqOrRev,
   parent=ReebChordSeq
 }
 \newglossaryentry{asubzero}{
   name={\ensuremath{a_0(\rhos)}},
   description={Element of $\Alg(n)$ associated to
  consistent set of Reeb chords $\rhos$},
   sort=arhossubzero,
   parent=algebrapmc
 }
 \newglossaryentry{aofrhos}{
   name={\ensuremath{a(\rhos)}},
   description={Element of $\Alg(\PMC)$ associated to
    set $\rhos$ of Reeb chords},
   sort=arhosz,
   parent=algebrapmc
 }
 \newglossaryentry{aofvecrho}{
   name={\ensuremath{a(\vec\rho)}},
   description={Product $a(\rho_1)\cdots a(\rho_n)$ where $\vec{\rho}=(\rho_1,\dots,\rho_n)$},
   sort=arhoszvec,
   parent=algebrapmc
 }
 \newglossaryentry{aofminusvecrho}{
   name={\ensuremath{a(-\vec\rho)}},
   description={Product $a(-\rho_1)\cdots a(-\rho_n)$ where $\vec{\rho}=(\rho_1,\dots,\rho_n)$},
   sort=arhoszvecminus,
   parent=algebrapmc
 }

 \newglossaryentry{uplusone}{
   name={\ensuremath{\uplus}},
   description={Join of abutting Reeb chords},
   sort=uplus,
   parent=algebrapmc
 }
 \newglossaryentry{uplus}{
%   name={\ensuremath{\uplus}},
   description={Join of composable sets of Reeb chords},
   sort=uplus,
   parent=uplusone
 }


%Heegaard diagrams:
 \newglossaryentry{heegaarddiagrams}
 {
   name={Heegaard diagrams},
   description={\nopostdesc}
 }

 \newglossaryentry{Heegaard}{
   name={\ensuremath{\Heegaard}},
   description={A bordered Heegaard diagram or pointed Heegaard diagram},
   sort=Heegaard,
   parent=heegaarddiagrams
 }
%  \newglossaryentry{BorderedHeegaard}{
% %   name={\ensuremath{\Heegaard}},
%    description={A bordered Heegaard diagram},
%    sort=Bordered,
%    parent=Heegaard
%  }
 \newglossaryentry{bSigma}{
   name={\ensuremath{\bSigma}},
   description={Compact Heegaard surface with one boundary component},
   sort=SigmaCpct,
   parent=heegaarddiagrams
}
\newglossaryentry{boundaryHD}{
  name={\ensuremath{\partial \HD}},
  description={Pointed matched circle appearing at the boundary of a
    bordered Heegaard diagram 
    $\HD$ (Lemma~\ref{lem:bdy-hd-is-pmc})},
  sort=dHD,
  parent=heegaarddiagrams
}
\newglossaryentry{Sigma}{
  name={\ensuremath{\Sigma}},
  description={Result of attaching a cylindrical end to $\bSigma$},
  sort=Sigma,
  parent=bSigma
  }
\newglossaryentry{oldSigma}{
  name={\ensuremath{\Sigma}},
  description={Heegaard surface for splitting of a closed manifold},
  sort=SigmaTwo
  parent=bSigma
  }

\newglossaryentry{homolclass}{
  name={\ensuremath{B}},
  description={A homology class in $\pi_2(\x,\y)$},
  sort=B,
  parent=heegaarddiagrams}
\newglossaryentry{homolclasshomolclass}{
  name={\ensuremath{[B]}},
  description={Element of $H_2(Y)$ represented by $B\in\pi_2(\x,\x)$},
  sort=Bhomolclass,
  parent=heegaarddiagrams}
\newglossaryentry{pitwo}{
  name={\ensuremath{\pi_2(\x,\y)}},
  description={Set of homology classes from $\x$ to $\y$ (with local
    multiplicity $0$ at $z$)},
  sort=pitwo,
  parent=heegaarddiagrams}
\newglossaryentry{pitwoBig}{
  name={\ensuremath{\protect\piBig(\x,\y)}},
  description={Set of homology classes from $\x$ to $\y$ with possibly
  non-zero local multiplicity at $z$; $\protect\piBig(\x,\y)\cong\ZZ\times\pi_2(\x,\y)$},
  sort=pitwoBig,
  parent=pitwo}
\newglossaryentry{pitwobdy}{
  name={\ensuremath{\pi_2^\bdy(\x,\y)}},
  description={Set of provincial homology classes from $\x$ to $\y$},
  sort=pitwobdy,
  parent=heegaarddiagrams}

\newglossaryentry{bdybdy}{
  name={\ensuremath{\bdy^\bdy(B)}},
  description={Portion of the
    boundary of $B$ contained in $\bdy\bSigma$},
  sort=bdyzbdy,
  parent=heegaarddiagrams}
\newglossaryentry{bdyalpha}{
  name={\ensuremath{\bdy^\alpha(B)}},
  description={Portion of the
    boundary of $B$ contained in $\balphas$},
  sort=bdyalpha,
  parent=heegaarddiagrams}
\newglossaryentry{bdybeta}{
  name={\ensuremath{\bdy^\beta(B)}},
  description={Portion of the
    boundary of $B$ contained in $\betas$},
  sort=bdybeta,
  parent=heegaarddiagrams}

\newglossaryentry{borderedmfld}{
  name={\ensuremath{(Y,\PMC,\phi)}},
  description={A bordered $3$-manifold},
  sort=YBordered,
  parent=heegaarddiagrams}
\newglossaryentry{YofHD}{
  name={\ensuremath{Y(\HD)}},
  description={The bordered $3$-manifold specified by a bordered
    Heegaard diagram $\HD$},
  sort=YofHD,
  parent=heegaarddiagrams}
\newglossaryentry{MorseFn}{
  name={\ensuremath{f}},
  description={A Morse function},
  sort=f,
  parent=heegaarddiagrams}
\newglossaryentry{Metric}{
  name={\ensuremath{g}},
  description={A Riemannian metric},
  sort=g,
  parent=heegaarddiagrams}



\newglossaryentry{betas}{
  name={\ensuremath{\betas}},
  description={Attaching circles in a closed or bordered
    Heegaard diagram corresponding to index $2$ critical points},
  sort=betas,
  parent=heegaarddiagrams}
% \newglossaryentry{oldbetas}{
% %  name={\ensuremath{\betas}},
%   description={Attaching circles in a pointed
%     Heegaard diagram for a closed manifold corresponding to index $2$ critical points},
%   sort=aabetas,
%   parent=betas}
\newglossaryentry{betai}{
  name={\ensuremath{\beta_i}},
  description={The $i\th$ curve in $\betas$},
  sort=betai,
  parent=betas}

\newglossaryentry{oalphas}{
  name={\ensuremath{\balphas}},
  description={Attaching circles and arcs in $\bSigma$ for a bordered
    Heegaard diagram corresponding to index $1$ critical points},
  sort=alphas,
  parent=heegaarddiagrams}
\newglossaryentry{alphas}{
  name={\ensuremath{\alphas}},
  description={Attaching circles in a pointed
    Heegaard diagram for a closed manifold corresponding to index $1$ critical points},
  sort=alphasa,
  parent=oalphas}
\newglossaryentry{noalphas}{
  name={\ensuremath{\alphas}},
  description={Curves in non-compact surface $\Sigma$ corresponding to $\balphas$},
  sort=alphas,
  parent=oalphas}
\newglossaryentry{alphasa}{
  name={\ensuremath{\balphas^a}},
  description={Attaching arcs among
  $\balphas$},
  sort=alphasarcs,
  parent=oalphas}
\newglossaryentry{noalphasa}{
  name={\ensuremath{\alphas^a}},
  description={Curves in $\Sigma$ corresponding to $\balphas^a$},
  sort=alphasarcsnon,
  parent=oalphas}
\newglossaryentry{alphasc}{
  name={\ensuremath{\alphas^c}},
  description={Attaching circles among
  $\balphas$},
  sort=alphascircles,
  parent=oalphas}
\newglossaryentry{alphaia}{
  name={\ensuremath{\balpha_i^a}},
  description={The $i\th$ curve in $\balphas^a$},
  sort=alphasaone,
  parent=oalphas}
\newglossaryentry{alphaic}{
  name={\ensuremath{\alpha_i^c}},
  description={The $i\th$ curve in $\alphas^c$},
  sort=alphascone,
  parent=oalphas}

\newglossaryentry{z}{
  name={\ensuremath{z}},
  description={Basepoint on $\bdy\overline{\Sigma}$ for a bordered
    Heegaard diagram or basepoint in $\Sigma$ for a closed Heegaard diagram},
  sort=z,
  parent=heegaarddiagrams}
% \newglossaryentry{oldz}{
%   description={Basepoint in $\Sigma$ in a closed Heegaard diagram},
%   sort=z,
%   parent=z}

\newglossaryentry{genx}{
  name={\ensuremath{\x}},
  description={A generator, a set of $g$ points in
    $\alphas\cap\betas$, one on each circle and at most one on each arc},
  sort=x,
  parent=heegaarddiagrams}
\newglossaryentry{genxi}{
  name={\ensuremath{x_i}},
  description={An element of the generator $\x$},
  sort=xi,
  parent=genx}
\newglossaryentry{generators}{
  name={\ensuremath{\S(\HD)}},
  description={The set of generators for the Heegaard diagram
    $\HD$},
  sort=generators,
  parent=heegaarddiagrams}
\newglossaryentry{generatorsTwo}{
  name={\ensuremath{\S(\Sigma,\alphas,\betas)}},
  description={Same as $\S(\HD)$ for $\HD=(\bSigma,\balphas,\betas,z)$},
  sort=generatorsTwo,
  parent=generators}
\newglossaryentry{generatorsS}{
  name={\ensuremath{\Gen(\HD,\s)}},
  description={The set of generators for the Heegaard diagram
    $\HD$ in the $\SpinC$-structure $\spinc$},
  sort=generatorsS,
  parent=generators}
\newglossaryentry{generatorsSrel}{
  name={\ensuremath{\Gen(\HD,\s^\rel)}},
  description={The set of generators for the Heegaard diagram
    $\HD$ in the relative $\SpinC$-structure $\s^\rel$},
  sort=generatorsSrel,
  parent=generators}
\newglossaryentry{generatorsUs}{
  name={\ensuremath{\protect\underline{\Gen}(\HD,\x_0)}},
  description={The set of generators for the twisted invariants for the Heegaard diagram
    $\HD$ based at the generator $\x_0$},
  sort=generatorsUs,
  parent=heegaarddiagrams}
\newglossaryentry{formale}{
  name={\ensuremath{e}},
  description={Formal variable used in twisted coefficients},
  sort=e,
  parent=heegaarddiagrams}

\newglossaryentry{ox}{
  name={\ensuremath{o(\x)}},
  description={Set of occupied $\alpha$-arcs in the
  generator $\x$},
  sort=ox,
  parent=heegaarddiagrams}
\newglossaryentry{osrhos}{
  name={\ensuremath{o(\SetS,\protect\vec{\rhos})}},
  description={Multi-set of $\alpha$-arcs obtained from multi-set $\SetS$ by deleting initial points of $\protect\vec{\rhos}$, adding terminal points of $\protect\vec{\rhos}$},
  sort=osr,
  parent=ox}
\newglossaryentry{osrhosint}{
  name={\ensuremath{o(\SetS,\protect\vec{\rhos}_{[1,i]})}},
  description={Same as $o(\SetS,\protect\vec{\rhos})$ but for initial
    segment $(\rho_1,\dots,\rho_i)$ of $\protect\vec{\rhos}$},
  sort=osrhosint,
  parent=ox}

\newglossaryentry{XofH}{
  name={\ensuremath{X(\HD)}},
  description={$\Field$-vector space spanned by $\Gen(\HD)$},
  sort=XofH,
  parent=heegaarddiagrams}
\newglossaryentry{XofHs}{
  name={\ensuremath{X(\HD,\spinc)}},
  description={$\Field$-vector space spanned by $\Gen(\HD,\spinc)$},
  sort=XofHs,
  parent=XofH}
\newglossaryentry{XofHUs}{
  name={\ensuremath{\protect\underline{X}(\HD,\x_0)}},
  description={$\Field$-vector space spanned by $\protect\underline{\Gen}(\HD,\x_0)$},
  sort=XofHUs,
  parent=heegaarddiagrams}

\newglossaryentry{concat}{
  name={\ensuremath{\ast}},
  description={Concatenation of homology classes corresponding to
    addition of domains},
  sort=concat,
  parent=heegaarddiagrams}

\newglossaryentry{szx}{
  name={\ensuremath{\s_z(\x)}},
  description={$\SpinC$-structure on $Y$ induced by the generator $\x$
  and basepoint $z$},
  sort=szxrel,
  parent=heegaarddiagrams}
\newglossaryentry{szxrel}{
  name={\ensuremath{\s_z^{\rel}(\x)}},
  description={Relative $\SpinC$-structure on $(Y,\bdy Y)$ induced by the generator $\x$
  and basepoint $z$},
  sort=szxrel,
  parent=heegaarddiagrams}

\newglossaryentry{epsilonxy}{
  name={\ensuremath{\epsilon(\x,\y)}},
  description={Obstruction to connecting $\x$ and $\y$ by a homology
    class; equal to $\s_z(\y)-\s_z(\x)$},
  sort=szxrel,
  parent=heegaarddiagrams}


\newglossaryentry{gluehomolclass}{
  name={\ensuremath{\glue}},
  description={Operation of gluing homology classes; also used for
    pregluing holomorphic curves},
  sort=gluehomol,
  parent=heegaarddiagrams}
\newglossaryentry{gluealongbdy}{
  name={\ensuremath{\cup_\bdy}},
  description={Gluing $3$-manifolds, Heegaard diagrams, etc.~along
    their boundaries},
  sort=glue,
  parent=heegaarddiagrams}

\newglossaryentry{nxB}{
  name={\ensuremath{n_x(B)}},
  description={Average multiplicity of $B$ near $x$},
  sort=nx,
  parent=heegaarddiagrams}
\newglossaryentry{nxboldB}{
  name={\ensuremath{n_\x(B)}},
  description={$\sum_{x_i\in \x}n_{x_i}(B)$},
  sort=nxbold,
  parent=heegaarddiagrams}

\newglossaryentry{aSW}{
  name={\ensuremath{a_{SW}, a_{SE}, a_{NW}, a_{NE}}},
  description={Small translates in $\Sigma\setminus(\alphas\cup\betas)$ of $a\in\alphas\cap\betas$},
  sort=aSW,
  parent=heegaarddiagrams}
\newglossaryentry{intnum}{
  name={\ensuremath{a\cdot b}},
  description={Intersection number or jittered intersection number of $a$ and $b$},
  sort=aSW,
  parent=heegaarddiagrams}

\newglossaryentry{Dz}{
  name={\ensuremath{D_z}},
  description={Region (component of
    $\bSigma\setminus(\balphas\cup\betas)$) adjacent to $z\in\bdy\bSigma$},
  sort=Dz,
  parent=heegaarddiagrams}



%Moduli:
\newglossaryentry{moduli}
{
  name={Moduli spaces},
  description={\nopostdesc}
}

\newglossaryentry{t}{
  name={\ensuremath{t}},
  description={Coordinate on $\RR$},
  sort=t,
  parent=moduli
}
\newglossaryentry{tsubi}{
  name={\ensuremath{t_i}},
  description={Height  ($t$-coordinate) of Reeb chord $\rho_i$},
  sort=tsubi,
  parent=t
}
\newglossaryentry{s}{
  name={\ensuremath{s}},
  description={Coordinate on $[0,1]$},
  sort=s,
  parent=moduli
}
\newglossaryentry{piSigma}{
  name={\ensuremath{\pi_\Sigma}},
  description={Projection $\Sigma\times[0,1]\times\RR\to \Sigma$},
  sort=piSigma,
  parent=moduli
}
\newglossaryentry{piD}{
  name={\ensuremath{\pi_\DD}},
  description={Projection $\Sigma\times[0,1]\times\RR\to [0,1]\times\RR$},
  sort=piD,
  parent=moduli
}


\newglossaryentry{plusinfty}{
  name={\ensuremath{+\infty}},
  description={End as $t\to\infty$ of $\Sigma\times[0,1]\times\RR$},
  sort=inftyplus,
  parent=moduli
}
\newglossaryentry{minusinfty}{
  name={\ensuremath{-\infty}},
  description={End as $t\to-\infty$ of $\Sigma\times[0,1]\times\RR$},
  sort=inftyminus,
  parent=moduli
}
\newglossaryentry{eastinfty}{
  name={\ensuremath{e\infty}},
  description={East infinity: end of $\Sigma\times[0,1]\times\RR$ at
    the puncture of $\Sigma$},
  sort=inftyeast,
  parent=moduli
}

\newglossaryentry{rhosubi}{
  name={\ensuremath{\rho_i}},
  description={A Reeb chord},
  sort=rhosubi,
  parent=moduli
}

\newglossaryentry{Partition}{
  name={\ensuremath{P}},
  description={A partition of the $e$ punctures of a decorated source $\Source$},
  sort=Partition,
  parent=moduli
}
\newglossaryentry{PartitionLength}{
  name={\ensuremath{\lvert P\rvert}},
  description={Number of parts of partition $P$},
  sort=PartitionLength,
  parent=Partition
}
\newglossaryentry{OrderedPartition}{
  name={\ensuremath{\protect\vec{P}}},
  description={An ordered partition of $e\infty$ punctures},
  sort=PartitionOrdered,
  parent=Partition
}
\newglossaryentry{Part}{
  name={\ensuremath{P_i}},
  description={A set of $e\infty$ punctures; a part in a
    partition or ordered partition},
  sort=PartitionPart,
  parent=Partition
}
\newglossaryentry{PartitionAssocChords}{
  name={\ensuremath{[P]}},
  description={Multi-sets of Reeb chords associated to partition $P$ of
    east punctures},
  sort=PartitionChords,
  parent=Partition
}
\newglossaryentry{PartitionOrderedAssocChords}{
  name={\ensuremath{[\protect\vec{P}]}},
  description={Sequence of multi-sets of Reeb chords associated to ordered partition $\protect\vec{P}$ of
    east punctures},
  sort=PartitionOrderedChords,
  parent=Partition
}

\newglossaryentry{PartitionEast}{
  name={\ensuremath{P_e}},
  description={A partition of the $e$ punctures of a bi-decorated source $\protect\biSource$},
  sort=PartitionEast,
  parent=moduli
}
\newglossaryentry{PartitionWest}{
  name={\ensuremath{P_w}},
  description={A partition of the $w$ punctures of a bi-decorated source $\protect\biSource$},
  sort=PartitionWest,
  parent=moduli
}


\newglossaryentry{ModSpaceOpenParam}{
  name={\ensuremath{\protect\tcM^B(\x,\y;\Source)}},
  description={Moduli space of curves with decorated source $\Source$
    asymptotic to $\x$ and $\y$},
  sort=ModuliSpace,
  parent=moduli
}
\newglossaryentry{ModSpaceCpctCpct}{
  name={\ensuremath{\protect\oocM^B(\x,\y;\Source)}},
  description={Space of holomorphic combs with preglued source
    $\Source$ connecting $\x$ to $\y$ in homology class $B$. Na\"ive compactification
  of $\cM^B(\x,\y;\Source)$},
  sort=AUnparamCpctCpct,
  parent=ModSpaceOpenParam
}
\newglossaryentry{ModSpaceCpct}{
  name={\ensuremath{\protect\ocM^B(\x,\y;\Source)}},
  description={Closure of $\cM^B(\x,\y;\Source)$ in
    $\oocM^B(\x,\y;\Source)$},
  sort=AUnparamCpctZ,
  parent=ModSpaceOpenParam
}
\newglossaryentry{ModSpaceUnorderedParam}{
  name={\ensuremath{\protect\tcM^B(\x,\y;\Source;{P})}},
  description={Moduli space of
  curves with decorated source $\Source$ asymptotic to $\x$ at
  $-\infty$ and $\y$ at $+\infty$, with partition of $e\infty$
  punctures ${P}$},
  sort=NotorderedParam,
  parent=ModSpaceOpenParam
}
\newglossaryentry{ModSpaceUnorderedCpctCpct}{
  name={\ensuremath{\protect\oocM^B(\x,\y;\Source;P)}},
  description={Space of holomorphic combs with preglued source
    $\Source$ connecting $\x$ to $\y$ in homology class $B$, respecting
    partition $P$ of east punctures. Na\"ive compactification
  of $\cM^B(\x,\y;\Source;P)$},
  sort=NotorderedUnparamCpctCpct,
  parent=ModSpaceOpenParam
}
\newglossaryentry{ModSpaceUnorderedCpct}{
  name={\ensuremath{\protect\ocM^B(\x,\y;\Source;P)}},
  description={Closure of $\cM^B(\x,\y;\Source;P)$ in
    $\oocM^B(\x,\y;\Source;P)$},
  sort=NotorderedUnparamCpctZ,
  parent=ModSpaceOpenParam
}
\newglossaryentry{ModSpaceUnorderedUnparam}{
  name={\ensuremath{\cM^B(\x,\y;\Source;{P})}},
  description={Quotient $\protect\tcM^B(\x,\y;\Source;{P})/\RR$},
  sort=NotorderedUnparam,
  parent=ModSpaceOpenParam
}
\newglossaryentry{ModSpaceOrderedParam}{
  name={\ensuremath{\protect\tcM^B(\x,\y;\Source;\protect\vec{P})}},
  description={Moduli space of
  curves with decorated source $\Source$ asymptotic to $\x$ at
  $-\infty$ and $\y$ at $+\infty$, with ordered partition  $\vec{P}$ of $e\infty$
  punctures},
  sort=OrderedParam,
  parent=ModSpaceOpenParam
}
\newglossaryentry{ModSpaceOrderedUnparam}{
  name={\ensuremath{\cM^B(\x,\y;\Source;\protect\vec{P})}},
  description={Quotient $\protect\tcM^B(\x,\y;\Source;\vec{P})/\RR$},
  sort=OrderedUnparam,
  parent=ModSpaceOpenParam
}
\newglossaryentry{ModSpaceOrderedCpct}{
  name={\ensuremath{\protect\ocM^B(\x,\y;\Source;\protect\vec{P})}},
  description={Compactification
  of the space $\cM^B(\x,\y;\Source;\vec{P})$, via holomorphic combs;
  the closure of
  $\cM^B(\x,\y;\Source;\vec{P})$ in $\oocM^B(\x,\y;\Source;\vec{P})$},
  sort=OrderedUnparamCpct,
  parent=ModSpaceOpenParam
}
\newglossaryentry{ModSpaceOpenBi}{
  name={\ensuremath{\protect\tcN(\protect\biSource)}},
  description={Moduli space of curves in $Z\times\RR\times[0,1]\times\RR$ with bi-decorated source $\protect\biSource$},
  sort=ModuliSpaceBi,
  parent=moduli
}
\newglossaryentry{ModSpaceBiOpenUnparam}{
  name={\ensuremath{\cN(\protect\biSource)}},
  description={Quotient $\tcN(\protect\biSource)/(\RR\times\RR)$},
  sort=ModuliSpaceBi,
  parent=ModSpaceOpenBi
}
\newglossaryentry{ModSpaceBiUnorderedParam}{
  name={\ensuremath{\protect\tcN(\protect\biSource;P_w,P_e)}},
  description={Subspace of $\tcN(\protect\biSource)$ with partitions
    $P_w$ / $P_e$ of west / east punctures},
  sort=ModuliSpaceUnorderedParam,
  parent=ModSpaceOpenBi
}
\newglossaryentry{ModSpaceBiUnorderedParamRDisc}{
  name={\ensuremath{\protect\tcN(\protect\biSource;P_e)}},
  description={Special case of $\tcN(\protect\biSource;P_w,P_e)$ where $P_w$
    is the discrete partition},
  sort=ModuliSpaceUnorderedParamRDisc,
  parent=ModSpaceOpenBi
}
\newglossaryentry{BdyModSpaceOrderedCpct}{
  name={\ensuremath{\bdy\protect\ocM^B(\x,\y;\Source)}},
  description={$\ocM^B(\x,\y\semico\Source\semico P)\setminus\cM^B(\x,\y\semico\Source\semico P)$},
  sort=BdyModSpace,
  parent=ModSpaceOpenParam
}
\newglossaryentry{ModSpaceEmbeddedOpen}{
  name={\ensuremath{\cM^B(\x,\y;\protect\vec\rhos)}},
  description={Open moduli space of embedded curves in homology class $B$ with asymptotics $\x$, $\y$ and $\vec{\rhos}$; counts of these moduli spaces are used to define $\CFDa$ and $\CFAa$},
  sort=ModSpaceEmbedded,
  parent=moduli
}
\newglossaryentry{ModSpaceEmbeddedCpct}{
  name={\ensuremath{\protect\ocM^B(\x,\y;\protect\vec\rhos)}},
  description={Compactified moduli space of embedded curves in homology class $B$ with asymptotics $\x$, $\y$ and $\vec{\rhos}$},
  sort=ModSpaceEmbeddedCpct,
  parent=moduli
}



\newglossaryentry{DecSource}{
  name={\ensuremath{\Source}},
  description={A decorated source},
  sort=SourceDec,
  parent=moduli
}
\newglossaryentry{SourceSurf}{
  name={\ensuremath{S}},
  description={Riemann surface underlying a decorated source $\Source$},
  sort=SourceSurf,
  parent=DecSource
}
\newglossaryentry{EofS}{
  name={\ensuremath{E(\Source)}},
  description={Set of east punctures of $\Source$},
  sort=E,
  parent=DecSource
}
\newglossaryentry{Eof}{
  name={\ensuremath{E}},
  description={Same as $E(\Source)$. Used when $\Source$ is clear from context},
  sort=EAlso,
  parent=DecSource
}

\newglossaryentry{biDecSource}{
  name={\ensuremath{\protect\biSource}},
  description={A bi-decorated source},
  sort=SourceDecbi,
  parent=moduli
}
\newglossaryentry{biSourceSurf}{
  name={\ensuremath{T}},
  description={Riemann surface underlying a bi-decorated source $\protect\biSource$},
  sort=SourceSurf,
  parent=biDecSource
}
\newglossaryentry{EofT}{
  name={\ensuremath{E(\protect\biSource)}},
  description={Set of east punctures of $\protect\biSource$},
  sort=ET,
  parent=biDecSource
}
\newglossaryentry{Eofbi}{
  name={\ensuremath{E}},
  description={Same as $E(\protect\biSource)$. Used when $\protect\biSource$ is clear from context},
  sort=ETAlso,
  parent=biDecSource
}
\newglossaryentry{WofT}{
  name={\ensuremath{W(\protect\biSource)}},
  description={Set of west punctures of $\protect\biSource$},
  sort=WT,
  parent=biDecSource
}
\newglossaryentry{Wofbi}{
  name={\ensuremath{W}},
  description={Same as $W(\protect\biSource)$. Used when $\protect\biSource$ is clear from context},
  sort=WTAlso,
  parent=biDecSource
}


\newglossaryentry{SigmaSymp}{
  name={\ensuremath{\omega_\Sigma}},
  description={Symplectic form on $\Sigma$ (fixed)},
  sort=SymplecticSigma,
  parent=moduli
}
\newglossaryentry{DSymp}{
  name={\ensuremath{\omega_\DD}},
  description={Standard symplectic form on $\DD$},
  sort=SymplecticD,
  parent=moduli
}

\newglossaryentry{SigmaCx}{
  name={\ensuremath{j_\Sigma}},
  description={Complex structure on $\Sigma$ (fixed)},
  sort=jSigma,
  parent=moduli
}
\newglossaryentry{DCx}{
  name={\ensuremath{j_\DD}},
  description={Standard complex structure on $\DD$},
  sort=jD,
  parent=moduli
}

\newglossaryentry{p}{
  name={\ensuremath{p}},
  description={Puncture of $\Sigma$ corresponding to $\bdy\overline{\Sigma}$},
  sort=p,
  parent=moduli
}
\newglossaryentry{Usubp}{
  name={\ensuremath{U_p}},
  description={Neighborhood of puncture $p$ of $\Sigma$},
  sort=U,
  parent=p
}
\newglossaryentry{pphi}{
  name={\ensuremath{\phi}},
  description={Identification of neighborhood $U_p$ of $p$
  with $S^1\times(0,\infty)$},
  sort=phi,
  parent=p
}

\newglossaryentry{Sigmae}{
  name={\ensuremath{\Sigma_{\widebar e}}},
  description={Closed Riemann surface obtained by filling puncture of
    $\Sigma$},
  sort=Sigmae,
  parent=bSigma
}

\newglossaryentry{u}{
  name={\ensuremath{u}},
  description={A holomorphic curve in $\Sigma\times[0,1]\times\RR$},
  sort=u,
  parent=moduli
}
\newglossaryentry{bracu}{
  name={\ensuremath{[u]}},
  description={Homology class of $u$},
  sort=bracu,
  parent=u
}
\newglossaryentry{capU}{
  name={\ensuremath{U}},
  description={A holomorphic comb},
  sort=Ucap,
  parent=moduli
}

\newglossaryentry{v}{
  name={\ensuremath{v}},
  description={A holomorphic curve in $Z\times\RR\times[0,1]\times\RR$},
  sort=v,
  parent=moduli
}
\newglossaryentry{uv}{
  name={\ensuremath{(u,v)}},
  description={A simple holomorphic comb},
  sort=uv,
  parent=moduli
}

\newglossaryentry{ev}{
  name={\ensuremath{ev}},
  description={Evaluation map $\cM^B(\x,\y;\Source;\protect\vec{P})\to\RR^E/\RR$},
  sort=ev,
  parent=moduli
}
\newglossaryentry{evq}{
  name={\ensuremath{ev_q}},
  description={Evaluation map at the puncture $q$, a map
    $\tcM^B(\x,\y;\Source;\protect\vec{P})\to\RR$ or $\tcN^B(\protect\biSource)\to\RR$},
  sort=evq,
  parent=ev
}
% \newglossaryentry{evqeast}{
%   name={\ensuremath{ev_q}},
%   description={Evaluation map at the puncture $q$, a map $\tcN^B(\protect\biSource)\to\RR$},
%   sort=evqeast,
%   parent=ev
% }
\newglossaryentry{evpq}{
  name={\ensuremath{ev_{p,q}}},
  description={Difference $\ev_p-\ev_q$},
  sort=evqp,
  parent=ev
}
\newglossaryentry{evpqcpct}{
  name={\ensuremath{\overline{ev}_{p,q}}},
  description={Extension of $\ev_{p,q}$ to $\oocM^B(\x,\y;\Source)$},
  sort=evqpcpct,
  parent=ev
}
\newglossaryentry{eveast}{
  name={\ensuremath{ev_e}},
  description={Evaluation map at the east punctures of $\protect\biSource$, a map $\tcN^B(\protect\biSource)\to\RR^{E(\protect\biSource)}$},
  sort=evqeasts,
  parent=ev
}
\newglossaryentry{evwest}{
  name={\ensuremath{ev_w}},
  description={Evaluation map at the west punctures of $\protect\biSource$, a map $\tcN^B(\protect\biSource)\to\RR^{W(\protect\biSource)}$},
  sort=evqwests,
  parent=ev
}

\newglossaryentry{PartialDiagonal}{
  name={\ensuremath{\Delta_P}},
  description={Partial diagonal $\{\,x_p=x_q \mid P_i\in P,\,\,p,q\in
    P_i\,\}$ associated to partition $P$},
  sort=Diagonal,
  parent=moduli
}

\newglossaryentry{indSource}{
  name={\ensuremath{\ind(B,\Source,P)}},
  description={Expected dimension of $\tcM^B(\x,\y;\Source;P)$},
  sort=indexSource,
  parent=moduli
}

\newglossaryentry{Euler}{
  name={\ensuremath{e(B)}},
  description={Euler measure of domain $B$},
  sort=Euler,
  parent=moduli
}

\newglossaryentry{tauR}{
  name={\ensuremath{\tau_R}},
  description={Translation of $\Sigma\times[0,1]\times\RR$ by $R\in\RR$},
  sort=tauR,
  parent=moduli
}

\newglossaryentry{REmodR}{
  name={\ensuremath{\RR^E/\RR}},
  description={Quotient of $\RR^E$ by simultaneous translation; target
  space for evaluation maps},
  sort=REmodR,
  parent=moduli
}
\newglossaryentry{preglue}{
  name={\ensuremath{\natural}},
  description={Pregluing of holomorphic curves; also used for gluing
    homology classes},
  sort=preglue,
  parent=moduli
}

\newglossaryentry{chiemb}{
  name={\ensuremath{\chi_{\emb}(B,\protect\vec{\rhos})}},
  description={Euler characteristic of embedded curve in homology
    class $B$ with asymptotics $\vec{\rhos}$, given by $\chi_{\emb}(B,\vec{\rhos})=
g+e(B)-n_\x(B)-n_\y(B)-\iota(\vec{\rhos})$},
  sort=chiemb,
  parent=moduli
}
\newglossaryentry{indemb}{
  name={\ensuremath{\ind(B,\protect\vec{\rhos})}},
  description={Expected dimension of moduli space of embedded curves in homology class $B$ with asymptotics $\vec{\rhos}$; $\ind(B,\vec{\rhos})=
e(B)+n_\x(B)+n_\y(B)+|\vec\rhos|+\iota(\vec{\rhos})$},
  sort=indemb,
  parent=moduli
}



\newglossaryentry{TypeDMod}
{
  name={Type $D$ modules},
  description={\nopostdesc},
  sort=TypeDMod
}
\newglossaryentry{IDofx}{
  name={\ensuremath{I_D(\x)}},
  description={Idempotent for $\CFDa$ for generator $\x$; $I_D(\x)=I([2k]\setminus o(\x))$},
  sort=IDofx,
  parent=TypeDMod
}
\newglossaryentry{CFD}{
  name={\ensuremath{\protect\CFDa(\HD)}},
  description={Type $D$ invariant associated in Section~\ref{sec:def-CFD} to bordered Heegaard diagram $\HD$},
  sort=CFDHD,
  parent=TypeDMod
}
\newglossaryentry{CFDspinc}{
  name={\ensuremath{\protect\CFDa(\HD,\spinc)}},
  description={Summand of $\CFDa(\HD)$ corresponding to $\SpinC$-structure $\spinc$},
  sort=CFDspincHD,
  parent=CFD
}
\newglossaryentry{CFDY}{
  name={\ensuremath{\protect\CFDa(Y)}},
  description={Type $D$ invariant $\CFDa(\HD)$ associated to any bordered Heegaard diagram $\HD$},
  sort=CFD,
  parent=TypeDMod
}
\newglossaryentry{CFDspincY}{
  name={\ensuremath{\protect\CFDa(Y,\spinc)}},
  description={Summand of $\CFDa(Y)$ corresponding to $\SpinC$-structure $\spinc$},
  sort=CFDaspinc,
  parent=CFDY
}
\newglossaryentry{tCFD}{
  name={\ensuremath{\protect\tCFDa(\HD,\x_0)}},
  description={Totally twisted variant of $\CFDa(\HD)$, with base
    generator $\x_0$},
  sort=CFDtwisted,
  parent=TypeDMod
}

\newglossaryentry{aBxy}{
  name={\ensuremath{a^B_{\x,\y}}},
  description={Coefficient of $\y$ in $\bdy x$ coming from
    homology class $B$},
  sort=aBxy,
  parent=TypeDMod
}
\newglossaryentry{axynoB}{
  name={\ensuremath{a_{\x,\y}}},
  description={Coefficient of $\y$ in $\bdy x$; the sum
    over $B$ of $a^B_{\x,\y}$},
  sort=axynoB,
  parent=aBxy
}

\newglossaryentry{DInvariance}
{
  name={Invariance of $\CFDa$},
  description={\nopostdesc},
  sort=TypeDModInv
}
\newglossaryentry{CFDJ}{
  name={\ensuremath{\protect\CFDa(\HD,\spinc;J)}},
  description={Module $\CFDa(\HD,\spinc)$ computed with respect to the
  almost complex structure $J$},
  sort=CFDJ,
  parent=DInvariance
}
\newglossaryentry{FJr}{
  name={\ensuremath{F^{J_r}}},
  description={Continuation map associated to path $J_r$ of almost
    complex structures},
  sort=FJr,
  parent=DInvariance
}

\newglossaryentry{ModCxStrSource}{
  name={\ensuremath{\protect\Mod^B(\x,\y;\Source;P;J)}},
  description={Moduli space of
  curves for $t$-dependent almost complex structure $J$ with decorated
  source $\Source$ asymptotic to $\x$ at
  $-\infty$ and $\y$ at $+\infty$, with partition of $e\infty$
  punctures ${P}$},
  sort=ModCxStrSource,
  parent=DInvariance
}
\newglossaryentry{ModCxStrEmb}{
  name={\ensuremath{\Mod^B(\x,\y; \vec{\rhos};J)}},
  description=
  {Open moduli space of embedded curves with respect to $t$-dependent
    complex structure $J$ in homology class $B$ with asymptotics $\x$, $\y$ and $\vec{\rhos}$},
  sort=ModCxStrEmb,
  parent=DInvariance
}
\newglossaryentry{ModTriSource}{
  name={\ensuremath{\cM^B(\x,\y,\Theta_o;\TSource)}},
  description={Moduli space of
  holomorphic triangles with decorated
  source $\TSource$ asymptotic to $\x$ at
  $v_{31}$, $\y$ at $v_{23}$ and $\Theta_o$ at $v_{12}$},
  sort=ModTriSource,
  parent=DInvariance
}

\newglossaryentry{ModTriSourcePP}{
  name={\ensuremath{\cM^B(\x,\y,\Theta_o;\TSource;\vec{P},\vec{P}^H)}},
  description={Subspace of $\tcM^B(\x,\y,\Theta_o;\TSource)$
    with ordered partition of east punctures $\vec{P}$ along $e_1$ and
  $\vec{P}^H$ along $e_2$},
  sort=ModTriSourcePP,
  parent=DInvariance
}
\newglossaryentry{ModTriSourcePPpd}{
  name={\ensuremath{\cM^B(\x,\y,\w_\pd^-;\TSource;\vec{P},\vec{P}^H)}},
  description={Moduli space of triangles with source $\TSource$
    asymptotic to partially diagonal generator $\w_\pd^-$ at
    $v_{12}$}, 
  sort=ModTriSourcePPw,
  parent=DInvariance
}
\newglossaryentry{ModTriSourcePPCpct}{
  name={\ensuremath{\protect\ocM^B(\x,\y,\Theta_o;\TSource;\protect\vec{P},\protect\vec{P}^H)}},
  description={Closure of $\protect\cM^B(\x,\y,\Theta_o;\TSource;\protect\vec{P},\protect\vec{P}^H)$ in $\protect\oocM^B(\x,\y,\Theta_o;\TSource;\protect\vec{P},\protect\vec{P}^H)$},
  sort=ModTriSourcePPzCpct,
  parent=DInvariance
}
\newglossaryentry{ModTriSourcePPCpctCpct}{
  name={\ensuremath{\protect\oocM^B(\x,\y,\Theta_o;\TSource;\protect\vec{P},\protect\vec{P}^H)}},
  description={Naive compactification of
    $\protect\cM^B(\x,\y,\Theta_o;\TSource;\protect\vec{P},\protect\vec{P}^H)$
    via combs},
  sort=ModTriSourcePPCpct,
  parent=DInvariance
}
\newglossaryentry{ModTriEmb}{
  name={\ensuremath{\Mod^B(\x,\y,\Theta; \vec{\rhos}) }},
  description={Moduli space of embedded
  triangles asymptotic to $\x$ at
  $v_{31}$, $\y$ at $v_{23}$, some $\Theta_o$ at $v_{12}$ and $\vec{\rhos}$
along $e_1$ and $e_2$},
  sort=ModTriSourceEmb,
  parent=DInvariance
}    
\newglossaryentry{ModTriEmbpd}{
  name={\ensuremath{\Mod^B(\x,\y,\w_\pd^-; \vec{\rhos},\vec{\rhos}^H) }},
  description={Moduli space of embedded
  triangles asymptotic to partially-diagonal generator $w_\pd^-$ at $v_{12}$, $\vec{\rhos}$
along $e_1$ and $\vec{\rhos}^H$ along $e_2$},
  sort=ModTriSourceEmbpd,
  parent=DInvariance
}    
\newglossaryentry{ModTriEmbRoneRtwo}{
  name={\ensuremath{\Mod^B(\x,\y,\Theta_o; \vec{\rhos}_1,\vec{\rhos}_2) }},
  description={Moduli space of embedded
  triangles asymptotic to $\x$ at
  $v_{31}$, $\y$ at $v_{23}$, $\Theta_{o}$ at $v_{12}$, $\vec{\rhos}_1$
  along $e_1$ and $\vec{\rhos}_2$ along $e_2$},
  sort=ModTriSourceEmbRoneRtwo,
  parent=DInvariance
}    
\newglossaryentry{ModVonetwo}{
  name={\ensuremath{\cM^B(\Theta_o,\w_\pd^+)}},
  description={Moduli space of holomorphic curves in $(\Sigma,\alphas^H,\alphas)$},
  sort=ModVonetwo,
  parent=DInvariance
}    
\newglossaryentry{ModVonetwoSource}{
  name={\ensuremath{\cM^B(\Theta_o,\w_\pd^+;\Source)}},
  description={Same as $\cM^B(\Theta_o,\w_\pd^+)$; used when we want
    to name the source},
  sort=ModVonetwo,
  parent=ModVonetwo
}    



\newglossaryentry{pdgen}{
  name={\ensuremath{w^\pm_\pd}},
  description={Positive / negative partially-diagonal generators},
  sort=wpm,
  parent=DInvariance
}    

\newglossaryentry{mumatching}{
  name={\ensuremath{\mu}},
  description={Matching between partially diagonal generators},
  sort=mumatching,
  parent=DInvariance
}    
\newglossaryentry{rhosofpdgens}{
  name={\ensuremath{\rhos_{\alphas}(\w^+_\pd,\w^-_\pd)}},
  description={Sequence of $\alpha$-Reeb chords associated to
    partially diagonal generators $\w^\pm_\pd$ and matching $\mu$},
  sort=rhosofpdgens,
  parent=DInvariance
}    
\newglossaryentry{rhosHofpdgens}{
  name={\ensuremath{\rhos_{\alphas^H}(\w^+_\pd,\w^-_\pd)}},
  description={Sequence of $\alpha^H$-Reeb chords associated to
    partially diagonal generators $\w^\pm_\pd$ and matching $\mu$},
  sort=rhosofpdgensH,
  parent=DInvariance
}    


\newglossaryentry{FaaHb}{
  name={\ensuremath{F_{\alphas,\alphas^H,\betas}}},
  description={Continuation map $\CFDa(\Sigma,\alphas^H,\betas,z)\to
\CFDa(\Sigma,\alphas,\betas,z)$ for a handleslide gotten by counting triangles},
  sort=FTriaaHb,
  parent=DInvariance
}

\newglossaryentry{TriangleDelta}{
  name={\ensuremath{\Delta}},
  description={A triangle (disk with three boundary punctures)},
  sort=Delta,
  parent=DInvariance
}
\newglossaryentry{TriangleEdges}{
  name={\ensuremath{e_1, e_2, e_3}},
  description={Edges of $\Delta$},
  sort=Edges,
  parent=TriangleDelta
}
\newglossaryentry{TriangleVertices}{
  name={\ensuremath{v_{12}, v_{23}, v_{13}}},
  description={Vertices of $\Delta$; $v_{ij}$ is adjacent to $e_i$
    and $e_j$},
  sort=Vertices,
  parent=TriangleDelta
}

\newglossaryentry{alphasH}{
  name={\ensuremath{\alphas^H}},
  description={$\alpha$-curves gotten by handlesliding $\alpha_1^a$
    over $\alpha_1^c$ and performing an appropriate isotopy},
  sort=alphasH,
  parent=DInvariance
}
\newglossaryentry{alphaicH}{
  name={\ensuremath{\alpha_i^{c,H}}},
  description={$i\th$ circle in $\alphas^H$; a small perturbation of
    $\alpha_i^c$ intersecting $\alpha_i^c$ in two points},
  sort=alphasH,
  parent=alphasH
}
\newglossaryentry{alphaiaH}{
  name={\ensuremath{\alpha_i^{a,H}}},
  description={$i\th$ arc in $\alphas^H$; for $i\geq 2$ a small perturbation of
    $\alpha_i^a$ intersecting $\alpha_i^a$ in one point; for $i=1$, a
    handleslide of $\alpha_1^a$ over $\alpha_1^c$, appropriately perturbed},
  sort=alphasH,
  parent=alphasH
}
\newglossaryentry{CircPtsH}{
  name={\ensuremath{\CircPts^H}},
  description={$\alphas^H\cap\bdy\overline{\Sigma}$},
  sort=aH,
  parent=alphasH
}

\newglossaryentry{alphasprime}{
  name={\ensuremath{\alphas^\prime}},
  description={Appropriately chosen small perturbation of $\alphas$},
  sort=alphasprime,
  parent=DInvariance
}
\newglossaryentry{alphaicprime}{
  name={\ensuremath{\alpha_i^{c,\prime}}},
  description={$i\th$ circle in $\alphas^\prime$, a small deformation
    of $\alpha_i^c$},
  sort=alphasprime,
  parent=alphasprime
}
\newglossaryentry{alphaiaprime}{
  name={\ensuremath{\alpha_i^{a,\prime}}},
  description={$i\th$ arc in $\alphas^\prime$, a small deformation of $\alpha_i^a$},
  sort=alphasprime,
  parent=alphasprime
}


\newglossaryentry{TSource}{
  name={\ensuremath{\TSource}},
  description={Decorated source for maps to $\Sigma\times\Delta$},
  sort=Tsource,
  parent=DInvariance
}

\newglossaryentry{Thetao}{
  name={\ensuremath{\Theta_o}},
  description={Top-graded generator for $(\Sigma,\alphas^H,\alphas)$
    with idempotent $I_D(o)$},
  sort=Thetao,
  parent=DInvariance
}
\newglossaryentry{pi2xyThetao}{
  name={\ensuremath{\pi_2(\x,\y,\Theta_o)}},
  description={Set of homology classes for $(\Sigma,\alphas,\alphas^H,\betas)$
    connecting $\x$, $\y$, and $\Theta_o$},
  sort=pi2xyThetao,
  parent=DInvariance
}

\newglossaryentry{IndTri}{
  name={\ensuremath{\ind(B,\TSource,P,P^H)}},
  description={Expected dimension of $\tcM^B(\x,\y,\Theta_o;\TSource;\vec{P},\vec{P}^H)$},
  sort=IndTri,
  parent=DInvariance
}

\newglossaryentry{xprime}{
  name={\ensuremath{\x'}},
  description={Nearest generator in $\Gen(\alphas^H,\betas)$ to $\x\in\Gen(\alphas,\betas)$},
  sort=xprime,
  parent=DInvariance
}

\newglossaryentry{smallTriClass}{
  name={\ensuremath{T_\x}},
  description={Canonical small triangle homology class in $\pi_2(\x,\x',\Theta_{o(\x)})$},
  sort=TriClass,
  parent=DInvariance
}

\newglossaryentry{starij}{
  name={\ensuremath{*_{ij}}},
  description={Operation of attaching a homology class at corner
    $v_{ij}$ of $\Delta$},
  sort=starij,
  parent=DInvariance
}

\newglossaryentry{bofB}{
  name={\ensuremath{b(B)}},
  description={Domain in $\pi_2(\x',\y)$ for the diagram $(\Sigma,\alphas^H,\betas)$ corresponding to
    domain $B\in\pi_2(\x,\y,\Theta_o)$, as in Lemma~\ref{lem:triple-pi2-decomp}},
  sort=bofB,
  parent=DInvariance
}



\newglossaryentry{TypeAMod}
{
  name={Type $A$ modules},
  description={\nopostdesc},
  sort=TypezAMod
}
\newglossaryentry{IAofx}{
  name={\ensuremath{I_A(\x)}},
  description={Idempotent for $\CFAa$ for generator $\x$; $I_A(\x)=I(o(\x))$},
  sort=IAofx,
  parent=TypeAMod
}
\newglossaryentry{CFA}{
  name={\ensuremath{\protect\CFAa(\HD)}},
  description={Type $A$ invariant associated in Section~\ref{sec:def-CFA} to bordered Heegaard diagram $\HD$},
  sort=CFAHD,
  parent=TypeAMod
}
\newglossaryentry{CFAspinc}{
  name={\ensuremath{\protect\CFAa(\HD,\spinc)}},
  description={Summand of $\CFAa(\HD)$ corresponding to $\SpinC$-structure $\spinc$},
  sort=CFAspincHD,
  parent=TypeAMod
}
\newglossaryentry{CFAY}{
  name={\ensuremath{\protect\CFAa(Y)}},
  description={Type $A$ invariant $\CFAa(\HD)$ associated to any bordered Heegaard diagram $\HD$},
  sort=CFA,
  parent=TypeAMod
}
\newglossaryentry{CFAspincY}{
  name={\ensuremath{\protect\CFAa(Y,\spinc)}},
  description={Summand of $\CFAa(Y)$ corresponding to $\SpinC$-structure $\spinc$},
  sort=CFAaspinc,
  parent=TypeAMod
}
\newglossaryentry{tCFA}{
  name={\ensuremath{\protect\tCFAa(\HD,\x_0)}},
  description={Totally twisted variant of $\CFAa(\HD)$, with base
    generator $\x_0$},
  sort=CFAtwisted,
  parent=TypeAMod
}
\newglossaryentry{monCFA}{
  name={\ensuremath{m_{n+1}}},
  description={$\Ainf$ products on $\CFAa$},
  sort=monCFA,
  parent=TypeAMod
}
\newglossaryentry{bdyCFA}{
  name={\ensuremath{\bdy(x)}},
  description={Alternate notation for $m_1(\x)$},
  sort=bdyCFA,
  parent=TypeAMod
}
\newglossaryentry{multCFA}{
  name={\ensuremath{\x\cdot a}},
  description={Alternate notation for $m_2(\x,a)$},
  sort=multCFA,
  parent=TypeAMod
}
\newglossaryentry{CFAJContMap}{
  name={\ensuremath{f^{J_r}_n}},
  description={$\Ainf$ chain homotopy equivalence on $\CFAa$ associated to
    change in almost complex structure},
  sort=fJrn,
  parent=TypeAMod
}

% \newglossaryentry{AInvariance}
% {
%   name={Invariance of $\CFAa$},
%   description={\nopostdesc},
%   sort=TypezAModInv
% }

\newglossaryentry{Pairing}
{
  name={The pairing theorem},
  description={\nopostdesc},
  sort=UPairing
}
\newglossaryentry{HDsubi}{
  name={\ensuremath{\HD_i=(\Sigma_i,\alphas_i,\betas_i,z)}},
  description={Provincially admissible Heegaard diagrams with $\bdy\HD_1=-\bdy\HD_2$},
  sort=abasicHDsubi,
  parent=Pairing
}
\newglossaryentry{pairingSigma}{
  name={\ensuremath{\Sigma,\alphas,\betas}},
  description={$\bSigma_1\cup_\bdy\bSigma_2$,
    $\balphas_1\cup_\bdy\balphas_2$ and $\betas_1\cup\betas_2$, respectively},
  sort=abasicNotation,
  parent=Pairing
}
\newglossaryentry{closedSource}{
  name={\ensuremath{\closedSource}},
  description={The pregluing $\SourceSub{1}\glue\SourceSub{2}$ of
    sources $\SourceSub{i}$ for curves in $\HD_i$},
  sort=closedSource,
  parent=Pairing
}
\newglossaryentry{MatchMod}{
  name={\ensuremath{\protect\tcMM^B(\x_1,\y_1,\SourceSub{1};\x_2,\y_2,\SourceSub{2})}},
  description={Matched moduli space, the fibered product over the
    evaluation maps $
  \tcM^{B_1}(\x_1,\y_1;\SourceSub{1})\times_{\ev_1=\ev_2}
  \tcM^{B_2}(\x_2,\y_2;\SourceSub{2})$},
  sort=ModMatched,
  parent=Pairing
}
\newglossaryentry{MatchModUnparam}{
  name={\ensuremath{\cMM^B(\x_1,\y_1,\SourceSub{1}\semico\x_2,\y_2,\SourceSub{2})}},
  description={Quotient $\tcMM^B(\x_1,\y_1,\SourceSub{1};\x_2,\y_2,\SourceSub{2})/\RR$},
  sort=ModMatchedaUnparam,
  parent=Pairing
}
\newglossaryentry{MatchModCpct}{
  name={\ensuremath{\protect\ocMM^B(\x_1,\y_1,\SourceSub{1}\semico\x_2,\y_2,\SourceSub{2})}},
  description={Compactification of $\cMM^B(\x_1,\y_1,\SourceSub{1}\semico\x_2,\y_2,\SourceSub{2})$},
  sort=ModMatchedaUnparamCpct,
  parent=Pairing
}
\newglossaryentry{MatchModEmb}{
  name={\ensuremath{\protect\tcMM{}^B(\x_1,\y_1\semico\x_2,\y_2)}},
  description={Embedded matched moduli space, union of matched moduli spaces with $\chi(\SourceSub{1}\glue\SourceSub{2})=\chi_\emb(B)$},
  sort=ModMatchedEmb,
  parent=Pairing
}
\newglossaryentry{MatchModEmbUnparam}{
  name={\ensuremath{\cMM{}^B(\x_1,\y_1\semico\x_2,\y_2)}},
  description={Quotient $\tcMM{}^B(\x_1,\y_1\semico\x_2,\y_2)/\RR$},
  sort=ModMatchedEmbUnparam,
  parent=Pairing
}
\newglossaryentry{TMatchMod}{
  name={\ensuremath{\protect\tcMM{}^B(T\semico\x_1,\y_1,\SourceSub{1}\semico
  \x_2,\y_2,\SourceSub{2})}},
  description={$T$-matched moduli space, the fibered product of moduli
    spaces $
  \tcM^{B_1}(\x_1,\y_1;\SourceSub{1})\times_{T\ev_1=\ev_2}
  \tcM^{B_2}(\x_2,\y_2;\SourceSub{2})$},
  sort=ModTMatched,
  parent=Pairing
}
\newglossaryentry{TMatchModUnparam}{
  name={\ensuremath{\cMM{}^B(T\semico\x_1,\y_1,\SourceSub{1}\semico
  \x_2,\y_2,\SourceSub{2})}},
  description={Quotient $\tcMM{}^B(T\semico\x_1,\y_1,\SourceSub{1}\semico
  \x_2,\y_2,\SourceSub{2})/\RR$},
  sort=ModTMatchedaUnparam,
  parent=Pairing
}
\newglossaryentry{TMatchModEmb}{
  name={\ensuremath{\protect\tcMM{}^B(T;\x_1,\y_1\semico\x_2,\y_2)}},
  description={Embedded $T$-matched moduli space, union of $T$-matched moduli spaces with $\chi(\SourceSub{1}\glue\SourceSub{2})=\chi_\emb(B)$},
  sort=ModTMatchedEmb,
  parent=Pairing
}
\newglossaryentry{TMatchModEmbUnparam}{
  name={\ensuremath{\cMM{}^B(T;\x_1,\y_1\semico\x_2,\y_2)}},
  description={Quotient $\tcMM{}^B(T;\x_1,\y_1\semico\x_2,\y_2)/\RR$},
  sort=ModTMatchedEmbUnparam,
  parent=Pairing
}

\newglossaryentry{psiMatchMod}{
  name={\ensuremath{\cMM{}^B(\psi\semico\x_1,\y_1,\SourceSub{1}\semico
  \x_2,\y_2,\SourceSub{2})}},
  description={Moduli space of $\psi$-matched pairs},
  sort=ModUpsiMatched,
  parent=Pairing
}
\newglossaryentry{psiMatchModEmb}{
  name={\ensuremath{\cMM{}^B(\psi;\x_1,\y_1\semico\x_2,\y_2)}},
  description={Union of $\psi$-matched moduli spaces with $\chi(\SourceSub{1}\glue\SourceSub{2})=\chi_\emb(B)$},
  sort=ModUpsiMatchedEmb,
  parent=Pairing
}

\newglossaryentry{geqTMatchMod}{
  name={\ensuremath{\protect\cMM{}^B(\geq T_0\semico\x_1,\y_1,\SourceSub{1}\semico
  \x_2,\y_2,\SourceSub{2})}},
  description={Union of $T$-matched moduli spaces for $T\geq T_0$},
  sort=ModTzgeqMatched,
  parent=Pairing
}

\newglossaryentry{tsicMod}{
  name={\ensuremath{\protect\cMM^B_\tsic(\x_1,\y_1,\SourceSub{1};\x_2,\y_2;\SourceSub{2})}},
  description={Moduli space of trimmed simple ideal-matched curves
    (modulo translation)},
  sort=Modztrim,
  parent=Pairing
}
\newglossaryentry{tsicModEmb}{
  name={\ensuremath{\protect\cMM^B_\tsic(\x_1,\y_1;\x_2,\y_2)}},
  description={Moduli space of embedded trimmed simple ideal-matched
    curves, given by the union $\bigcup_{\{\SourceSub{1},\SourceSub{2}\mid
  \chi(\SourceSub{1}\glue\SourceSub{2})=\chi_\emb(B)\}}
\cMM^B_\tsic(\x_1,\y_1,\SourceSub{1};\x_2,\y_2;\SourceSub{2})$},
  sort=Modztrim,
  parent=Pairing
}


\newglossaryentry{MatchIndSrc}{
  name={\ensuremath{\ind(B_1, \SourceSub{1}; B_2,\SourceSub{2})}},
  description={Expected dimension of $\tcMM{}_0^B(\x_1,\y_1,\SourceSub{1};\x_2,\y_2,\SourceSub{2})$},
  sort=ModInd,
  parent=Pairing
}

\newglossaryentry{TimeSpace}{
  name={\ensuremath{T(U)}},
  description={Time parameter space of a holomorphic comb $U$},
  sort=TimeSpace,
  parent=Pairing
}
\newglossaryentry{Tdilation}{
  name={\ensuremath{T}},
  description={Dilation parameter, a positive real number},
  sort=Tdilation,
  parent=Pairing
}
\newglossaryentry{psidilation}{
  name={\ensuremath{\psi(t)}},
  description={Dilation function interpolating between $T_1$ and
    $T_2$. Also used for grading refinement data},
  sort=Tpsidilation,
  parent=Pairing
}

\newglossaryentry{Tdiff}{
  name={\ensuremath{\partial_T(\x_1\times\x_2)}},
  description={$T$-deformed differential, on $\CFa(T;\HD_1,\HD_2)$},
  sort=bdyT,
  parent=Pairing
}

\newglossaryentry{Tcont}{
  name={\ensuremath{F_{T_1,T_2}}},
  description={Chain homotopy equivalence from $\CFa(T_1;\HD_1,\HD_2)$
    to $\CFa(T_2;\HD_1,\HD_2)$ from counting $\psi$-matched curves},
  sort=FToneTtwo,
  parent=Pairing
}

\newglossaryentry{phicorresp}{
  name={\ensuremath{\varphi}},
  description={Correspondence between the punctures of $U_1$ and $U_2$
  in an ideal-matched holomorphic comb},
  sort=phicorresp,
  parent=Pairing
}

\newglossaryentry{CFTimeDilated}{
  name={\ensuremath{\CFa(T;\HD_1,\HD_2)}},
  description={Analogue of $\CFa(\HD_1\cup_\bdy\HD_2)$ computed using
    $T$-matched holomorphic curves},
  sort=CFTimeDilated,
  parent=Pairing
}


\newglossaryentry{Torus}
{
  name={Manifolds with torus boundary},
  description={\nopostdesc},
  sort=vTorus
}
\newglossaryentry{AlgTorus}{
  name={\ensuremath{\Alg(\Torus)}},
  description={Algebra $\Alg(\Torus,0)$ associated to the unique
    pointed matched circle for a torus in the central ($i=0$) $\SpinC$
    structure},
  sort=AlgTorus,
  parent=Torus
}
\newglossaryentry{torusalphaarcs}{
  name={\ensuremath{\alpha_1^a,\alpha_2^a}},
  description={$\alpha$-arcs in a Heegaard diagram with torus
    boundary, labeled as in Section~\ref{sec:torus-algebra}},
  sort=alphaarcs,
  parent=Torus
}
\newglossaryentry{torusidempotents}{
  name={\ensuremath{\iota_0,\iota_1}},
  description={Indecomposable idempotents in $\Alg(\Torus)$, labeled
    so that $\iota_0$ corresponds to $\alpha_1^a$ occupied on type $A$
  side (unoccupied on type $D$ side)},
  sort=idempotents,
  parent=Torus
}
\newglossaryentry{torusreebgens}{
  name={\ensuremath{\rho_1,\rho_2,\rho_3,\rho_{12},\rho_{23},\rho_{123}}},
  description={Non-idempotent basic generators for $\Alg(\Torus)$},
  sort=rhos,
  parent=Torus
}

\newglossaryentry{torusbiggrgp}{
  name={\ensuremath{\bigGroup}},
  description={$\bigGroup(4)$, the unrefined grading group
    for the torus algebra},
  sort=grgpabig,
  parent=Torus
}
\newglossaryentry{torussmallgrgp}{
  name={\ensuremath{\smallGroup}},
  description={$\smallGroup(\Torus)$, the refined grading group
    for the torus algebra},
  sort=grgpasmall,
  parent=Torus
}
\newglossaryentry{torusbiggrgpelt}{
  name={\ensuremath{(m;a,b,c)}},
  description={Element of $\bigGroup$},
  sort=grgpeltbig,
  parent=Torus
}
\newglossaryentry{torussmallgrgpelt}{
  name={\ensuremath{(m;a,b)}},
  description={Element of $\smallGroup$},
  sort=grgpeltsmall,
  parent=Torus
}
\newglossaryentry{coeffmap}{
  name={\ensuremath{D_{I}}},
  description={Coefficient map %for type $D$ structure over
    over
    $\Alg(\Torus)$ corresponding to $I\subset \{1,2,3\}$; or
    generalized coefficient maps for $I\subset \{0,1,2,3\}$ a cyclic interval}, 
  sort=DsubI,
  parent=Torus
}

\newglossaryentry{HDSolidTori}{
  name={\ensuremath{\HD_{-1}, \HD_0, \HD_\infty}},
  description={Standard Heegaard diagrams for $-1$-, $0$- and
    $\infty$-framed solid tori, respectively}, 
  sort=HDSolidTori,
  parent=Torus
}

\newglossaryentry{AGrading}{
  name={\ensuremath{\protect\AGrading(\PMC)}},
  description={$\smallGroup(\PMC)\times\ZZ$; the extra $\ZZ$ is the Alexander factor},
  sort=AGrading,
  parent=Torus
}
\newglossaryentry{Ags}{
  name={\ensuremath{\protect\Ags}},
  description={Enhanced grading of domains in presence of knot, $(g(B),n_{w}(B)-n_{z}(B))\!\in\protect\AGrading$},
  sort=gs,
  parent=AGrading
}
\newglossaryentry{Agr}{
  name={\ensuremath{\protect\Agr}},
  description={Enhanced grading on $\CFD$ in presence of knot given by
    $\Ags(B)\cdot \APeriodics(\x_0)$ for $B\in\pi_2(\x,\x_0)$},
  sort=gs,
  parent=AGrading
}
\newglossaryentry{AGradingD}{
  name={\ensuremath{\protect\AGradingD}},
  description={$\protect\AGrading$-set for $\CFD^-({\mathcal H},z,w)$ given by
  $\protect\AGrading/\protect\APeriodics(\x_0)$},
  sort=AGradingD,
  parent=AGrading
}
\newglossaryentry{APeriodics}{
  name={\ensuremath{\protect\APeriodics(\x_0)}},
  description={$\Ags(\pi_2(\x_0,\x_0))\subset \protect\AGrading$},
  sort=APeriodics,
  parent=AGrading
}


\newglossaryentry{U}{
  name={\ensuremath{U}},
  description={Formal variable used in knot Floer homology},
  sort=U,
  parent=Torus
}
\newglossaryentry{AgrUx}{
  name={\ensuremath{\protect\Agr(Ux)}},
  description={$(\lambda^{-2},-1)\cdot\Agr(x)$},
  sort=grading,
  parent=U
}

\newglossaryentry{DblyPtdHD}{
  name={\ensuremath{(\Sigma,\alphas,\betas,w,z)}},
  description={A doubly pointed Heegaard diagram for a knot in a $3$-manifold},
  sort=knotHD,
  parent=Torus
}
\newglossaryentry{knotGen}{
  name={\ensuremath{\Gen_K}},
  description={Generators for knot Floer complex},
  sort=knotGen,
  parent=Torus
}
\newglossaryentry{knotCxminus}{
  name={\ensuremath{\CFKm(K)}},
  description={Knot Floer complex, a filtered complex generated over $\Field[U]$ by $\Gen_K$},
  sort=knotCxminus,
  parent=Torus
}
\newglossaryentry{gknotCxminus}{
  name={\ensuremath{\gCFKm(K)}},
  description={Associated graded complex to $\CFKm(K)$},
  sort=gknotCxminus,
  parent=knotCxminus
}


\newglossaryentry{knotCxHat}{
  name={\ensuremath{\protect\CFKa(K)}},
  description={$U=0$ specialization of $\CFKm(K)$, a filtered complex generated over $\Field$ by $\Gen_K$},
  sort=knotCxzHat,
  parent=Torus
}
\newglossaryentry{gknotCxHat}{
  name={\ensuremath{\protect\gCFKa(K)}},
  description={Associated graded complex to $\CFKa(\HD)$},
  sort=gknotCx,
  parent=knotCxHat
}
\newglossaryentry{knotCxAssocGr}{
  name={\ensuremath{C}},
  description={Shorthand for $\gCFKa(K)$},
  sort=gzknotCx,
  parent=knotCxHat
}
\newglossaryentry{knotCxAssocGrSummand}{
  name={\ensuremath{C(r)}},
  description={Summand $\gCFKa(\HD,r)$ of $\gCFKa(K)$ in Alexander
    grading $r$},
  sort=gzzaSummand,
  parent=knotCxHat
}
\newglossaryentry{knotCxAssocGrPos}{
  name={\ensuremath{C(\geqo s)}},
  description={$\bigoplus_{r\geq s} C(r)$},
  sort=gzzazPosSummand,
  parent=knotCxHat
}
\newglossaryentry{knotCxAssocGrNeg}{
  name={\ensuremath{C(\leqo s)}},
  description={$\bigoplus_{r\leq s} C(r)$},
  sort=gzzazNegSummand,
  parent=knotCxHat
}
\newglossaryentry{bdyi}{
  name={\ensuremath{\bdy^i}},
  description={Map $C(r)\rightarrow C(r+i)$ defined by counting holomorphic disks $\phi$ with
    $n_{z}(\phi)=-i$ and $n_{w}(\phi)=0$ if $i\leq 0$, and $n_{z}(\phi)=0$
    and $n_{w}(\phi)=i$ if $i\geq 0$},
  sort=gzzbdyi,
  parent=knotCxHat
}
\newglossaryentry{bdyw}{
  name={\ensuremath{\bdy_w}},
  description={$\sum_{i\geq 0} \partial^i$},
  sort=gzzbdyw,
  parent=knotCxHat
}
\newglossaryentry{bdyz}{
  name={\ensuremath{\bdy_z}},
  description={$\sum_{i\leq 0} \partial^i$},
  sort=gzzbdyz,
  parent=knotCxHat
}

\newglossaryentry{knotHminus}{
  name={\ensuremath{\HFKm(K)}},
  description={Knot Floer homology, homology of $\gCFKm(K)$},
  sort=knotHminus,
  parent=Torus
}
\newglossaryentry{knotHhat}{
  name={\ensuremath{\protect\HFKa(K)}},
  description={Homology of $\gCFKa(K)$},
  sort=knotHzhat,
  parent=Torus
}

\newglossaryentry{Alexander}{
  name={\ensuremath{A}},
  description={Alexander depth (filtration)},
  sort=A,
  parent=Torus
}
\newglossaryentry{Maslov}{
  name={\ensuremath{M}},
  description={Maslov grading on knot Floer complex},
  sort=M,
  parent=Torus
}
\newglossaryentry{Naslov}{
  name={\ensuremath{N}},
  description={Renormalized Maslov grading on knot Floer complex. $N=M-2A$},
  sort=N,
  parent=Torus
}

\newglossaryentry{tau}{
  name={\ensuremath{\tau}},
  description={The tau invariant from knot Floer homology},
  sort=tau,
  parent=Torus
}

\newglossaryentry{knotBorderedmA}{
  name={\ensuremath{\CFAm(\HD,z,w)}},
  description={Type $A$ variant of bordered knot Floer complex},
  sort=knotzCxAm,
  parent=Torus
}
\newglossaryentry{knotBorderedaA}{
  name={\ensuremath{\protect\CFAa(\HD,z,w)}},
  description={$U=0$ specialization of $\CFAm(\HD,z,w)$},
  sort=knotzCxAza,
  parent=Torus
}
\newglossaryentry{knotBorderedmD}{
  name={\ensuremath{\CFDm(\HD,z,w)}},
  description={Type $D$ variant of bordered knot Floer complex},
  sort=knotzCxDm,
  parent=Torus
}
\newglossaryentry{knotBorderedaD}{
  name={\ensuremath{\protect\CFDa(\HD,z,w)}},
  description={$U=0$ specialization of $\CFDm(\HD,z,w)$},
  sort=knotzCxDza,
  parent=Torus
}

\newglossaryentry{Cvert}{
  name={\ensuremath{\Cvert}},
  description={Vertical complex of a $\ZZ$-filtered, $\ZZ$-graded
    chain complex over $\Field[U]$},
  sort=Cvert,
  parent=Torus
}
\newglossaryentry{Chor}{
  name={\ensuremath{\Chor}},
  description={Horizontal complex of a $\ZZ$-filtered, $\ZZ$-graded
    chain complex over $\Field[U]$},
  sort=Chor,
  parent=Torus
}

\newglossaryentry{Hvert}{
  name={\ensuremath{\Hvert}},
  description={Vertical complex of a $\ZZ$-filtered, $\ZZ$-graded
    chain complex over $\Field[U]$},
  sort=Hvert,
  parent=Torus
}
\newglossaryentry{Hhor}{
  name={\ensuremath{\Hhor}},
  description={Horizontal complex of a $\ZZ$-filtered, $\ZZ$-graded
    chain complex over $\Field[U]$},
  sort=Hhor,
  parent=Torus
}

\newglossaryentry{Wi}{
  name={\ensuremath{W^i}},
  description={Summand of $\CFDa(\HD)$ (for $\HD$ as in
    Section~\ref{sec:CFK-to-CFD}) corresponding to idempotent $i$},
  sort=Wi,
  parent=Torus
}
\newglossaryentry{WiDecomp}{
  name={\ensuremath{\bigoplus_{s\in\frac{1}{2}\ZZ}W^i_s}},
  description={Decomposition of $W^i$ according to a grading function $S$},
  sort=WiDecomp,
  parent=Torus
}


\newglossaryentry{nframing}{
  name={\ensuremath{n}},
  description={The framing parameter in
    Section~\ref{sec:CFK-to-CFD}, a large positive integer},
  sort=n,
  parent=Torus
}
\newglossaryentry{cconst}{
  name={\ensuremath{c}},
  description={Constant $c$ such that exterior generators $\y$ have
    $|S(\y)|\leq c$},
  sort=c,
  parent=Torus
}


\newglossaryentry{VectZeroS}{
  name={\ensuremath{V^0_s}},
  description={$C(s)$},
  sort=VectZero,
  parent=Torus
}
\newglossaryentry{VectOneS}{
  name={\ensuremath{V^1_s}},
  description={$C(\leq s+\frac{n-1}{2})$ if $s\leq
    -n/4$; $\Field$ if $|s|< n/4$; and
        $C(\geq s-\frac{n-1}{2})$ if $s\geq n/4$},
  sort=VectOneS,
  parent=Torus
}
\newglossaryentry{VectZero}{
  name={\ensuremath{V^0}},
  description={$\bigoplus_{s\in\ZZ} V^0_s$},
  sort=VectZero,
  parent=VectZeroS
}
\newglossaryentry{VectOne}{
  name={\ensuremath{V^1}},
  description={$\bigoplus_{s\in\ZZ+\frac{n+1}{2}}V^1_s$},
  sort=VectOne,
  parent=VectOneS
}
\newglossaryentry{Vect}{
  name={\ensuremath{V}},
  description={$V^0\oplus V^1$},
  sort=Vectzz,
  parent=Torus
}

% \newglossaryentry{Wect}{
%   name={\ensuremath{W=W^0\oplus W^1}},
%   description={Vector space for type $D$ structure $\CFDa(\HD(n))$},
%   sort=Vectzz,
%   parent=Torus
% }


\newglossaryentry{HDforK}{
  name={\ensuremath{(\Sigma_0,\alphas_0,\betas_0,z,w)}},
  description={Doubly-pointed Heegaard diagram for $K\subset S^3$},
  sort=HDforK,
  parent=Torus
}
\newglossaryentry{HDforKstab}{
  name={\ensuremath{\HD_K\coloneqq(\Sigma,\alphas,\betas,z,w)}},
  description={Doubly-pointed Heegaard diagram for $K$ obtained by
    stabilizing the diagram $(\Sigma_0,\alphas_0,\betas_0,z,w)$},
  sort=HDforKstab,
  parent=Torus
}
\newglossaryentry{betag}{
  name={\ensuremath{\beta_g}},
  description={New $\beta$-circle in $\HD_K$ meeting $\alpha_g$ in a
    single point},
  sort=betag,
  parent=HDforKstab
}
\newglossaryentry{alphag}{
  name={\ensuremath{\alpha_g}},
  description={New $\alpha$-circle in $\HD_K$, contained in the new handle},
  sort=alphag,
  parent=HDforKstab
}
\newglossaryentry{HDofn}{
  name={\ensuremath{\HD(n)\coloneqq(\Sigma,\alpha_1^a,\alpha_2^a,\alpha_1,\dots,\alpha_{g-1},\betas)}},
  description={Bordered Heegaard diagram for $S^3\setminus\nbd(K)$ with
    framing $n$, coming from $\HD_K$},
  sort=HDofn,
  parent=Torus
}

\newglossaryentry{GenK}{
  name={\ensuremath{\Gen_K}},
  description={Set of generators for $\CFKa(\HD_K)$},
  sort=GenK,
  parent=Torus
}
\newglossaryentry{Genn}{
  name={\ensuremath{\Gen(n)}},
  description={Set of generators for $\CFDa(\HD(n))$},
  sort=Genn,
  parent=Torus
}

\newglossaryentry{xiWind}{
  name={\ensuremath{\{x_i\}_{i=-\frac{n}{2}}^{i=\frac{n}{2}}}},
  description={Intersections between $\beta_g$ and
    $\alpha_1^a\cup\alpha_2^a$, contained in winding region},
  sort=xiWind,
  parent=Torus
}
\newglossaryentry{xiWindBold}{
  name={\ensuremath{\{\x_i\}_{i=-\frac{n}{2}}^{i=\frac{n}{2}}}},
  description={Generators of $\CFDa(\HD(n))$ corresponding to
    generator $\x\in\Gen_K$},
  sort=xiWindBold,
  parent=Torus
}


\newglossaryentry{Winding}{
  name={\ensuremath{\Winding}},
  description={The winding region},
  sort=Winding,
  parent=Torus
}

\newglossaryentry{BsubZero}{
  name={\ensuremath{B_0}},
  description={Generator for periodic domains in $\HD(n)$, with local
    multiplicities $(0,1,1-n,-n)$ in regions $(0,1,2,3)$},
  sort=HDzBsubZero,
  parent=Torus
}

\newglossaryentry{AlexGrFun}{
  name={\ensuremath{S}},
  description={Function $\Gen(\HD)\rightarrow \OneHalf\ZZ$
    characterized by Equations~\eqref{eq:DefOfS}
    and~\eqref{eq:SNormalization}. Also used for source of holomorphic
  curves},
  sort=HDzBsubZero,
  parent=Torus
}

\newglossaryentry{phik}{
  name={\ensuremath{\phi_k}},
  description={Distinguished homology class in winding region connecting $x_k$ to
    $x_{k-1}$ with multiplicity $+1$ at regions $2$ and $3$},
  sort=phik,
  parent=Torus
}
\newglossaryentry{psik}{
  name={\ensuremath{\psi_k}},
  description={Distinguished homology class in winding region connecting $x_{k-1}$ to
    $x_{k}$ with multiplicity $0$ at regions $2$ and $3$},
  sort=psik,
  parent=Torus
}




\newglossaryentry{Bimodules}
{
  name={Bimodules and change of framing},
  description={\nopostdesc},
  sort=zBimodules
}
% \newglossaryentry{psiacts}{
%   name={\ensuremath{(Y,\phi)\psi}},
%   description={Action of mapping class $\psi$ on bordered $3$-manifold
%   $(Y,\phi)$ given by $(Y,\phi)\psi=(Y,\phi\circ\psi)$},
%   sort=psiacts,
%   parent=Bimodules
% }
\newglossaryentry{CFDApsi}{
  name={\ensuremath{\lsub{\Alg(\PMC)}\protect\CFDAa(\psi)_{\Alg(\PMC)}}},
  description={Type \DAm\ bimodule associated to mapping class $\psi$},
  sort=CFDApsi,
  parent=Bimodules
}
\newglossaryentry{mCFDA}{
  name={\ensuremath{m_{i,1,j}(a_1,\dots,a_i,\x,b_1,\dots,b_j)}},
  description={$\Ainf$ bimodule structure on $\CFDAa$},
  sort=mCFDA,
  parent=CFDApsi
}
\newglossaryentry{CFAAId}{
  name={\ensuremath{\protect\CFAAa(\Id)_{\Alg(\PMC),\Alg(-\PMC)}}},
  description={Type \AAm\ bimodule associated to the identity map of
    $F(\PMC)$; tensoring with this turns type $D$ invariants into type
  $A$ invariants},
  sort=CFzAAId,
  parent=Bimodules
}
\newglossaryentry{mCFAA}{
  name={\ensuremath{m_{1,i,j}(\x;a_1,\dots,a_i;,b_1,\dots,b_j)}},
  description={$\Ainf$ bimodule structure on $\CFAAa(\Id_\PMC)$},
  sort=mCFAAa,
  parent=CFAAId
}

\newglossaryentry{CFDDId}{
  name={\ensuremath{\lsub{\Alg(\PMC),\Alg(-\PMC)}\protect\CFDDa(\Id)}},
  description={Type \DDm\ bimodule associated to the identity map of
    $F(\PMC)$; tensoring with this turns type $A$ invariants into type
  $D$ invariants},
  sort=CFzDDId,
  parent=Bimodules
}
\newglossaryentry{CFDDIdbdy}{
  name={\ensuremath{\bdy}},
  description={Differential on $\CFDDa(\Id_\PMC)$ given by Equation~\eqref{eq:dd-id-diff}},
  sort=bdy,
  parent=CFDDId
}
\newglossaryentry{ModRS}{
  name={\ensuremath{M_{R,S}}},
  description={Bimodule with commuting right actions of $R$ and $S$},
  sort=MRS,
  parent=Bimodules
}
\newglossaryentry{RSMod}{
  name={\ensuremath{\lsub{R,S}M}},
  description={Bimodule with commuting left actions of $R$ and $S$},
  sort=MRS,
  parent=Bimodules
}
\newglossaryentry{abHD}{
  name={\ensuremath{\HD=(\overline{\Sigma},\overline\alphas,\betas,\arcz)}},
  description={Arced bordered Heegaard diagram. Also used for other
    kinds of Heegaard diagrams},
  sort=abHD,
  parent=Bimodules
}
\newglossaryentry{bdyLR}{
  name={\ensuremath{\bdy_L, \bdy_R}},
  description={Left and right boundaries of $\bSigma$, $Y$ or $\HD$},
  sort=bdyLR,
  parent=Bimodules
}
\newglossaryentry{PMCLR}{
  name={\ensuremath{\PMC_L, \PMC_R}},
  description={Left and right boundaries of $\HD$, i.e.,
    $\PMC_L=\bdy_L\HD$ and $\PMC_R=\bdy_R\HD$},
  sort=PMCLR,
  parent=Bimodules
}
\newglossaryentry{phiLR}{
  name={\ensuremath{\phi_L, \phi_R}},
  description={Homeomorphisms $\phi_L\co F(\PMC_L)\to\bdy_LY$ and
    $\phi_R\co F(\PMC_R)\to\bdy_RY$ specified by a bordered Heegaard
    diagram for $Y$},
  sort=phiLR,
  parent=Bimodules
}
\newglossaryentry{FLR}{
  name={\ensuremath{F_L, F_R}},
  description={Surfaces $F(\PMC_L)$ and $F(\PMC_R)$},
  sort=FLR,
  parent=Bimodules
}
\newglossaryentry{UpsilonofHD}{
  name={\ensuremath{\Upsilon(\HD)}},
  description={Strongly based mapping class associated to arced
    bordered Heegaard diagram $\HD$},
  sort=UpsilonofHD,
  parent=Bimodules
}
\newglossaryentry{MCGzero}{
  name={\ensuremath{\MCG_0}},
  description={Strongly based mapping class group},
  sort=phiofHD,
  parent=Bimodules
}
\newglossaryentry{BimGens}{
  name={\ensuremath{\S(\HD)}},
  description={The set of generators for the arced bordered Heegaard diagram
    $\HD$},
  sort=generators,
  parent=Bimodules}
\newglossaryentry{taumu}{
  name={\ensuremath{\tau_\mu}},
  description={Dehn twist of the standard torus around its meridian},
  sort=taumu,
  parent=Bimodules}
\newglossaryentry{taulambda}{
  name={\ensuremath{\tau_\lambda}},
  description={Dehn twist of the standard torus around its longitude},
  sort=taulambda,
  parent=Bimodules}
\newglossaryentry{pqrsgens}{
  name={\ensuremath{\mathbf{p},\mathbf{q},\mathbf{r},\mathbf{s}}},
  description={Generators for type \DAm\ invariants of $\tau_\mu^{\pm
      1}$, $\tau_\lambda^{\pm 1}$, with idempotents specified by
    Equation~\eqref{eq:pqrsIdems}},
  sort=pqrs,
  parent=Bimodules}
\newglossaryentry{oLxoRx}{
  name={\ensuremath{o^L(\x),o^R(\x)}},
  description={Set of $\alpha^L$ arcs and of $\alpha^R$ arcs occupied by
    $\x$, respectively},
  sort=oLxoRx,
  parent=Bimodules}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "InvPairing"
%%% End: 

